One-Shot Imitation Learning with Invariance Matching for Robotic Manipulation

Learning a single universal policy that can perform a diverse set of manipulation tasks is a promising new direction in robotics. However, existing techniques are limited to learning policies that can only perform tasks that are encountered during training, and require a large number of demonstrations to learn new tasks. Humans, on the other hand, often can learn a new task from a single unannotated demonstration. In this work, we propose the Invariance-Matching One-shot Policy Learning (IMOP) algorithm. In contrast to the standard practice of learning the end-effector's pose directly, IMOP first learns invariant regions of the state space for a given task, and then computes the end-effector's pose through matching the invariant regions between demonstrations and test scenes. Trained on the 18 RLBench tasks, IMOP achieves a success rate that outperforms the state-of-the-art consistently, by 4.5% on average over the 18 tasks. More importantly, IMOP can learn a novel task from a single unannotated demonstration, and without any fine-tuning, and achieves an average success rate improvement of $11.5\%$ over the state-of-the-art on 22 novel tasks selected across nine categories. IMOP can also generalize to new shapes and learn to manipulate objects that are different from those in the demonstration. Further, IMOP can perform one-shot sim-to-real transfer using a single real-robot demonstration.

==> backup/note.tex <==
% $\mathcal{I}(a, s)$ includes the points that have the invariant position within the end-effector frame under different instantiations of action $a$. 
% \todo{add a visual illustration.}
% Intuitively, $\mathcal{I}(a, s)$ is composed of the region that describes the action and thereby binds the action $a$ onto these semantic elements, \emph{e.g.}, pixels, or points. In doing so, action $a$ can be transferred from $s$ to $x$ through finding the \emph{invariance correspondence}  $\mathcal{C}(a, s, x)$ as in Definition~\ref{def:invariance-corr}. 
% $\mathcal{C}(a, s, x)$ captures the point-level mapping with the minimal pairwise distance in the end-effector frame.
% Therefore, if $\mathcal{C}(a, s, x)$ is given, the end-effector pose $a'$ in state $x$ can be analytically solved by $\min_{X_{a'}} \sum_{(p, q) \in \mathcal{C}(a, s, x)} \parallel X^{-1}_{a} \cdot p  -  X^{-1}_{a'} \cdot q \parallel$ using the least square method~\citep{huang1986least}.  



% Similar to the pioneering work by \citet{duan2017one}, we assume each query state $s^{q}$ can be routed to a support state $s_i^{sup} \in \tau$ where we denote $s^{q}$ as the state in actual interactions and $s_i^{sup}$ as states in demonstrations. However, unlike the simplistic setting where each state is a colored block \citep{duan2017one}, $s^q$ and $s_i^{sup}$ are high-dimensional point clouds. 
% With this assumption that a match between $s^{q}$ and $s_i^{sup}$ can be established, we simplify the one-shot policy from $\pi(a | s, \tau)$ to $\pi(a | s^q,  (s^{sup}_i, a_i, s_{i+1}))$. We focus on the prediction of the 6-DoF end-effector pose in $a \in \mathcal{A}$, as the binary prediction of gripper state and collision avoidance can be modeled with existing one-shot classification methods. 


% To approach these questions, we first conceptually categorize the actions. For $a \in \mathcal{A}$, we define $\mathcal{T}(a, s)$ as the instantiation of $a$ in state $s$. For example, if $a$ is the action of holding a cup in state $s$, then $\mathcal{T}(a, x)$ is that of holding a cup in a different state $x$. We assume  $\mathcal{T}(a, x)=\varnothing$ if state $x$ does not include the corresponding action.

% \begin{proposition}
% A match can be established between states $s$ and $x$ if $\mathcal{T}(a, s) \neq \varnothing$ and $\mathcal{T}(a, x) \neq \varnothing$, where $\exists \tau \in \mathcal{D}$ such that $(s, a) \subseteq \tau$ or $(x, a) \subseteq \tau$.
%  \label{prop:match-state}
% \end{proposition}

% As shown in Proposition~\ref{prop:match-state}, the conceptual definition of $\mathcal{T}(a, s)$ gives us a tangible understanding of matched states, \textit{i.e.}, two states can be matched when they expect the same type of action. In light of this, we arrive at an action-driven definition for invariance in Definition~\ref{def:invariance-ps}, where we use $X_a \in \mathbb{R}^{4\times 4}$ to denote the homogeneous transformation equivalent to the 6-DoF end-effector pose of $a$, $p \in s$ to denote a point in homogeneous coordinate in the point cloud of $s$, and $X^{-1}_a \cdot p$ to denote a point whose coordinate transformed to the end-effector frame. 



% In Algorithm~\ref{alg:train}, we compute the pointwise probability estimation $\widehat{\mathbf{P}}[p \in \mathcal{I}(a, s)], \forall p \in s$ and the pairwise probability $\widehat{\mathbf{P}}[(p, q) \in \mathcal{C}(a, s, x)], \forall p \in \mathcal{I}(a, s), \forall q \in x$ in line 5 and 7. The binary mask $b$ is computed from the given $\mathcal{I}(a, s)$ during training in line 6. We adopt the RvS (RL via supervised learning) paradigm similar to \citet{chen2021decision} and use focal loss between the probability estimation and given $\mathcal{I}(a, s)$ and $\mathcal{C}(a, s, x)$. It is worth noting that we assume the availability of $\mathcal{I}$, $\mathcal{C}$, and a dataset $\mathcal{D}_{pair}$ of matched state pairs in Algorithm~\ref{alg:train}. We detail their construction in Section~\ref{sec:impl}. In Algorithm~\ref{alg:inference}, we use $C$ to denote the $\widehat{\mathbf{P}}[(p, q) \in \mathcal{C}(a, s^{sup}_i, s^q)]$ in line 3, we use $P_{s^{sup}_i} \in \mathbb{R}^{3\times K}$ and $P_{s^q} \in \mathbb{R}^{3\times M}$ to denote the points in $s^{sup}_i$ and $s^q$. $P_{s^{sup}_i}[b] \in \mathbb{R}^{3\times I}$ denotes the points in the estimated \textit{invariance point set} of $s^{sup}_i$. With the soft assignment matrix $C$, the optimization problem in line 4 can be solved using the least square method proposed by \citet{huang1986least}. As shown in Definition~\ref{def:invariance-corr}, the result $[\begin{smallmatrix} R & t \\ 0 & 1 \\ \end{smallmatrix}]$ correspondences to $X_{a^q} \cdot X_a^{-1}$, from which $X_{a^q}$ can be recovered in line 5.




==> modules.backup/0.preamble.tex <==
\usepackage{booktabs, multirow}
\usepackage{amssymb}% http://ctan.org/pkg/amssymb
\usepackage{pifont}% http://ctan.org/pkg/pifont
\usepackage{subfig}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
\DeclareMathOperator*{\argmin}{argmin} 
\DeclareMathOperator*{\argmax}{argmax} 
\newcommand{\round}[1]{\ensuremath{\lfloor#1\rceil}}

\newcommand{\dhruv}[1]{\textcolor{blue}{(dhruv: #1)}}

\newcommand{\todo}[1]{{\color{red}{#1}}}
\newcommand{\new}[1]{{\color{orange}{#1}}} % text that recently added 
\newenvironment{nalign}{
    \begin{equation}
    \begin{aligned}
}{
    \end{aligned}
    \end{equation}
    \ignorespacesafterend
}

\definecolor{darkgreen}{rgb}{0,0.5,0}
\definecolor{darkyellow}{RGB}{153,153,0}
\definecolor{darkred}{rgb}{0.5,0,0}

==> modules.backup/1.head.tex <==


%\title{One-Shot Imitation Learning with Invariance Matching}
\title{One-Shot Imitation Learning with Invariance Matching for Robotic Manipulation}

% You will get a Paper-ID when submitting a pdf file to the conference system
\author{Author Names Omitted for Anonymous Review. Paper-ID 141}


==> modules.backup/2.abstract.tex <==
\begin{abstract}
Learning a single universal policy that can perform a diverse set of manipulation tasks is a promising new direction in robotics. However, existing techniques are limited to learning policies that can only perform tasks that are encountered during training, and require a large number of demonstrations to learn new tasks. Humans, on the other hand, often can learn a new task from a single unannotated demonstration. In this work, we propose the Invariance-Matching One-shot Policy Learning (IMOP) algorithm. In contrast to the standard practice of learning the end-effector's pose directly, IMOP first learns invariant regions of the state space for a given task, and then computes the end-effector's pose through a correspondence of invariant regions between demonstrations and test scenes. Trained on the 18 \textit{\textbf{RLBench}} tasks, IMOP achieves a success rate that outperforms the state-of-the-art consistently, by $4.5\%$ on average over the 18 tasks. More importantly, IMOP can learn a novel task from a single unannotated demonstration, and without any fine-tuning, and achieves an average success rate improvement of $11.5\%$ over the state-of-the-art on 22 novel tasks selected across nine categories. IMOP can also generalize to new shapes and learn to manipulate objects that are different from those in the demonstration. Further, IMOP can 
perform one-shot sim-to-real transfer using a single real-robot demonstration. 
% \todo{reminder: mention real robot exp in intro and/or abstract}
\end{abstract}

==> modules.backup/3.introduction.tex <==
\section{Introduction}
\label{sec:intro}

Multi-Task Learning (MTL) is a recent type of learning technique where a policy is trained to perform multiple tasks. With the recent advances in computer vision architectures~\citep{han2022survey}, a popular MTL strategy in robotics is to acquire a multi-task control policy through imitation learning from visual demonstrations~\citep{gervet2023act3d, goyal2023rvt, shridhar2023perceiver, xian2023chaineddiffuser}. These methods achieved impressive results in performing challenging manipulation tasks in unstructured 3D environments, such as RLBench~\citep{james2020rlbench}. However, these methods rely on the assumption that training and testing share the same set of tasks.
Moreover, training such policies on new tasks requires hundreds of demonstrations~\citep{goyal2023rvt}, which results in the catastrophic forgetting of old tasks~\citep{kirkpatrick2017overcoming}.

%The primary objective of robot learning is to develop systems capable of solving diverse manipulation tasks in unconstrained 3D environments. The robot should be able to learn new tasks without long system interaction time. With the recent advances in deep learning architectures~\citep{han2022survey}, a popular strategy is to acquire a multi-task robotic control policy through imitation learning from visual demonstration~\citep{shridhar2023perceiver, goyal2023rvt, gervet2023act3d, xian2023chaineddiffuser}. These methods achieved impressive results in challenging 3D manipulation task sets such as RLBench~\citep{james2020rlbench}. However, the success of these methods relies on the assumption that the same set of tasks is shared between training and testing. Moreover, training such policies requires hundreds of demonstrations for each task~\citep{goyal2023rvt}, which means a long system interaction time when learning new tasks and the risk of catastrophic forgetting~\citep{kirkpatrick2017overcoming}. That being said, these methods are not able to adeptly generalize to novel tasks after training.


To address these issues, one-shot imitation learning aims to learn on a set of {\it base tasks} and generalize to {\it novel tasks} given only a single demonstration for each novel task and without re-training. However, existing methods rely on strong assumptions, such as requiring the novel tasks to be limited variations of the same base tasks~\citep{xu2022prompting}, requiring the base and novel tasks to have the same object setup~\citep{dasari2021transformers}, only generalizing specific actions on certain categories of objects with known 3D models~\citep{biza2023one}, or operating in simple 2D planar environments~\citep{duan2017one}. Moreover, most recent works focus on applying general popular techniques, e.g., transformers and diffusion models, to one-shot imitation settings, without taking advantage of the particular structure of robotic manipulation tasks~\citep{dasari2021transformers, mandi2022towards, xu2022prompting, xu2023hyper}. %None of the existing methods develops a one-shot imitation learner for 3D robotic manipulation tasks. 


Therefore, a key question here is: can robots learn a manipulation policy that not only performs well on base tasks but also generalizes to novel unseen tasks using a single demonstration and without any fine-tuning? To this end, we propose IMOP (\textbf{I}nvariance \textbf{M}atching \textbf{O}ne-shot \textbf{P}olicy Learning), a new algorithm that not only outperforms the state-of-the-art on the standard 18 tasks of RLBench ($69.6\%$ average overall success rate compared to $65.1\%$ for the state-of-the-art~\citep{gervet2023act3d}), but also generalizes to 22 novel tasks with a single demonstration and without any fine-tuning ($41.3\%$ average success rate compared to $29.8\%$ for the state-of-the-art).  The 22 novel tasks are selected across nine categories and are substantially different from the base tasks in terms of objects and task goals~\citep{guhur2023instruction, james2020rlbench}. Moreover, we find that IMOP also generalizes to substantial shape variations, and can manipulate new objects that are different from those in the demonstration. 



Instead of learning the desired end-effector's pose directly, IMOP learns key {\it invariant 
% visited state 
regions} of each task, and finds pairwise correspondences between the invariant regions in a one-shot demonstration and in a given test scene. The pairwise correspondences are used to analytically compute the desired end-effector's pose in the test scene from the least-squares solution of a point-set registration problem. The invariant region is defined as a set of 3D points whose coordinates remain invariant across semantically equivalent scenes when viewed in the end-effector's frame. We devise an unsupervised procedure to automatically estimate invariant regions in offline demonstrations of base tasks. The estimated invariant regions are then used as pseudo ground truth to train three neural networks, one that learns invariant regions, another network that finds pairwise correspondences between invariant regions, and a third network that learns to find semantically equivalent scenes in a one-shot demonstration and in a test scene. 
%Trained on base tasks, IMOP demonstrates the ability to discover invariant regions on novel tasks, thereby achieving the one-shot generalization to novel tasks.

To summarize, our contributions are threefold. First, we propose IMOP, a one-shot imitation learning algorithm for robotic manipulation that learns a single universal policy that is not only successful on base tasks, but can also generalize to novel tasks using a single unannotated demonstration. Second, we propose the concept of invariant regions for manipulation tasks and design an unsupervised procedure to estimate invariant regions in offline demonstrations. %, which provides the data support of our invariance matching one-shot policy learning; 
Finally, we present a thorough empirical study of the performance and generalization ability of IMOP on a diverse set of tasks.


==> modules.backup/4.related_work.tex <==


\section{Related Work}
\label{sec:related_work}


\textbf{Learning robotic manipulation from demonstrations.} Learning manipulation policies from offline visual demonstrations has gained increasing attention following the rapid improvement of vision models~\citep{dosovitskiy2020image}. Prior works such as Transporter networks~\citep{zeng2021transporter} and CLIPort~\citep{shridhar2022cliport} learned simple pick-and-place tasks in a 2D planar setting. C2F-ARM~\citep{james2022coarse} and PerAct~\citep{shridhar2023perceiver} extend the control capacity to the 3D space with 6-DoF but learn a separate policy for each single task. More recently, RVT~\citep{goyal2023rvt}, Hiveformer~\citep{guhur2023instruction}, Act3D~\citep{gervet2023act3d}, and  ChainedDiffuser~\citep{xian2023chaineddiffuser} learned a multi-task policy from demonstrations of multiple tasks. Yet, these prior approaches can only perform tasks that were seen during training and cannot generalize to novel tasks upon inference. Training these models also requires hundreds of demonstrations per task. Instead, this work aims to develop a multi-task policy that not only performs well on seen tasks but also generalizes to novel tasks given a single demonstration.

\textbf{One-shot imitation learning. } Traditional imitation learning considers learning a policy for a single task with many expert trajectories provided for this particular task. 
One-shot imitation learning aims to learn from demonstrations of a set of base tasks and generalize to novel tasks using a single trajectory per new task without further training. \citet{duan2017one} trained a one-shot imitator that generalizes to simple task variations in a 2D stacking environment. \citet{finn2017one} used the same setting in the context of  meta-learning. \citet{dasari2021transformers, xu2022prompting} and \citet{mandi2022towards} trained transformer-based one-shot imitators, such as encoding expert trajectories as prompts. \citet{biza2023one} achieved one-shot generalization for grasping tasks where 3D models of the objects are available. \citet{xu2023hyper} trained adaptation layers through hyper-networks. Yet, none of these prior works considered 6D manipulation tasks in the context of one-shot learning. 
 Moreover, recent works focus on applying existing techniques, such as transformers and adaptation layers, to one-shot imitation settings, but did not investigate the inherent task structure of robotic manipulation. 
In contrast, this work proposes a one-shot imitation learner for 6D  manipulation by discovering invariant regions of each task.

% not assume similarity between base and novel tasks or enforce the same object setup, and discover invariant regions inherent to each given task. 
% are limited in the scope of generalization, \textit{e.g.}, require novel tasks to be similar varieties of base tasks, share the same object setup between base and novel tasks, or use a simple planar environment \todo{(reference)}.


\textbf{Invariance in deep learning. } Incorporating invariance into deep learning models has been shown to drastically increase data efficiency and generalization~\citep{brandstetter2021geometric, cohen2016group, cohen2018spherical, van2020mdp}. Existing approaches can be divided into two categories. One is to design operators to build invariance into the networks, \emph{e.g.}, using spherical convolutions to guarantee an invariant output given a rotated input~\citep{cohen2016group}. The other one is to design data augmentation strategies such that the network is trained to predict invariant outputs~\citep{lyle2020benefits}.
% Dhruv change: The other is to design data augmentation strategies so the networks are trained to predict invariant outputs from inputs of specific transformations 
Our approach subscribes to this line of methods, and applies the concept of invariance to robotic manipulation. But instead of building operators or relying on augmentations, we train neural networks that can predict invariant state regions.

% Contrary to existing work, we discover the invariant region for robotic manipulation tasks. We estimate the invariant regions within offline demonstrations and train neural networks to find invariance in novel tasks instead of building specific operators. 



==> modules.backup/5.method.tex <==
\section{One-shot Imitation with Invariance Matching}
\label{sec:method}

\begin{figure}
  \includegraphics[width=\linewidth]{assets/mot.drawio.png}
  % \vspace{-2em}
  \caption{Example of a pick-and-place task executed by a real Kuka robot after observing a single demonstration and without any re-training. 
  The correspondences between estimated invariant regions of the 3D point cloud in the demonstration and in the test scene are visualized in \textcolor{darkred}{red} lines. The invariant regions are predicted by a neural network, trained offline.}
  \label{fig:motivating}
\end{figure}



\subsection{A Motivating Example}

%Figure~\ref{fig:motivating} demonstrates the one-shot generalization of our method IMOP in the context of sim-to-real transfer.
%IMOP is able to generalize to novel tasks or perform sim-to-real transfer, given a single demonstration without any re-training. 
Figure~\ref{fig:motivating} illustrates an example from our experiments where a Kuka robot is tasked with  picking up an object (pear) and placing it in a bowl, using a single demonstration of picking up and placing a different object (duck) in a different position. 
At the core of IMOP lies the capacity to estimate invariant regions of the given task. By finding a correspondence of invariant regions in the demonstration and in the test scene, the demonstrated actions can be transferred to the test scene. In this example, the invariant regions are: (1) a set of 3D points on the surfaces of the pear and the duck where contact with the fingertips occurs, and (2), a set of 3D points from the bowl's point cloud that capture its spherical concave shape. 
The invariant regions of the 3D point cloud are learned offline from unannotated demonstrations, on various objects and tasks.

%We outline the next sections as follows. In Section~\ref{sec:formulation}, we formulate the one-shot manipulation learning problem. In Section~\ref{sec:task-inv-space}, we define the invariant region and invariance correspondence and explain how to derive target end-effector pose from these two structures.  In Section~\ref{sec:offline-inv-e}, we explain how to estimate invariant regions in the offline dataset, \textit{i.e.}, prepare training data for learning invariance estimator and matcher as neural networks. In Section~\ref{sec:algo} and \ref{sec:impl-detail}, we explain the IMOP algorithm for training and evaluation, and implementation details, such as network architectures. 




% closely overlap the pick and place targets




\subsection{Formulation of One-shot Manipulation Learning Problem}
\label{sec:formulation}



\begin{figure*}
  \includegraphics[width=\textwidth]{assets/rlbench.drawio.png}
  % \vspace{-2em}
  \caption{Examples of tasks, and object-level generalization in various trials. After training on base tasks, IMOP is evaluated on novel tasks that are substantially different from the base tasks. Every learned task is evaluated in multiple trials, each with different object layouts and orientations. For each novel task, only one recorded trajectory is given as a demonstration. We summarize the performance of IMOP on both base and novel tasks in Section~\ref{sec:exp-base} and \ref{sec:exp-novel}. Further, we study the ability of IMOP to generalize to new objects beyond those in the demonstrations in Section~\ref{sec:exp-beyond-demo}.}
  % \todo{Consider linking this figure in the motivating example and the beginning of the exp section}}
  \label{fig:rlbench}
\end{figure*}


We use $\mathbf{T}$ to denote a set of manipulation tasks $\{\textrm{Task}_1,\textrm{Task}_2,\dots,\textrm{Task}_{N_\textrm{tasks}}\}$. Each manipulation task $\textrm{Task}_i\in \mathbf{T}$ is performed in a Markov Decision Process (MDP) represented by 5-tuple $\mathcal{M}_i = (\mathcal{S}, \mathcal{A}, \mathbf{P}, R_i, \mu_i)$, wherein $\mathcal{S}$ and $\mathcal{A}$ are state and action spaces, $\mathbf{P}:\mathcal{S}\times\mathcal{A}\mapsto\mathcal{S}$ is a state transition probability, $R_i: \mathcal{S}\mapsto\mathbb{R}$ denotes a reward function associated with task $\textrm{Task}_i$, and $\mu_i$ is the initial state distribution of $\textrm{Task}_i$. $\mathbf{T}$ is composed of a set of base tasks, denoted by $\mathbf{T}^{base}$, and a set of novel tasks, denoted by $\mathbf{T}^{novel}$. Thus, $\mathbf{T} = \mathbf{T}^{base} \cup \mathbf{T}^{novel}$. During training, a dataset $\mathcal{D}_{base} = \{(\textrm{Task}_{k_i}, s_{i}, a_{i}, s_{i}')\}_{i=1}^{|\mathcal{D}_{base}|}$ of examples is provided for the base tasks, where $\textrm{Task}_{k_i}\in \mathbf{T}^{base}$ is the label of the base task in example $i$, $a_i$ is a demonstrated action in state $s_i$, and $s{_i}'$ is the resulting next state. $|\mathcal{D}_{base}|$ denotes the number of provided examples. %$\mathcal{D}_{base}$ is collected from successful demonstrations on a set of base tasks $\mathbf{T}^{base}$. 
%$\mathcal{D}_{base}$ does not include reward because $R_t$ is a binary success indicator function in the manipulation setting and only returns 1 at the last transition of a successful episode and 0 otherwise. 
The underlying reward function of each task is unknown and is not used in this work.
During testing, only one successful trajectory $\tau_i = \{(\textrm{Task}_i,s^{new}_t, a^{new}_t, s^{new}_{t+1})\}_{t=1}^{|\tau_i|}$ is provided to the robot for a novel $\textrm{Task}_i\in \mathbf{T}^{novel}$, where $|\tau_i|$ denotes the number of transitions. 
% $\tau_i = \{(\textrm{Task}_i,s^{new}_t, a^{new}_t, s^{new}_{t+1})\}_{t=1}^{H_{i}}$ is provided to the robot for a novel $\textrm{Task}_i\in \mathbf{T}^{novel}$, where $H_{i}$ denotes the number of transitions. 
%We refer to $\tau_i$ as the demonstration trajectory for $\textrm{Task}_i$. %Each task $t$ comes from $\mathbf{T}^{base} \cup \mathbf{T}^{novel}$, where $\mathbf{T}^{novel}$ represents a set of novel tasks that is disjoint to $\mathbf{T}^{base}$.  
The goal is to learn a one-shot universal policy $\pi(s,\tau_i)$, which is a multi-task policy that returns an action $a$ in new state $s$ given a single demonstrated trajectory $\tau_i$ of the desired novel skill. $\tau_i$ is provided in an environment that is different from the one in which $\pi$ is tested. 
%, and does not require any finetuning.

A state $s \in \mathcal{S}$ is a raw 3D point cloud of the entire scene, including the robot. Each point $p_i \in s, i \in \{1, ..., |s|\}$, where $|s|$ denotes the number of points in state $s$, is represented in homogeneous coordinates. An action $a \in \mathcal{A}$ is the desired (i.e., target) 6D pose of the robot's end-effector, along with the desired state of the gripper. To execute an action, low-level robot movements are generated using off-the-shelf motion planners.
% \dhruv{This needs to change, T is 16 numbers} 
More precisely, we define actions as 18-dimensional vectors $a = (T, \lambda)$, wherein $T \in \mathbb{R}^{4\times4}$ denotes the target end-effector pose given as a homogeneous matrix and is referred to as action pose, and $\lambda$ denotes two binary values that indicate whether the gripper is open or closed, and whether collisions are allowed or not.

%For example, RLBench~\citep{james2020rlbench} uses an 8-dimensional action, including the 6-DoF end-effector pose (3-DoF for translation and 3-DoF for rotation), two binary indicators for gripper state (open or close, whether to allow collision). We write $a = (T_a, \lambda_a)$ to decompose action into two components, where $T_a \in \mathbb{R}^{4\times4}$ denotes the target end-effector pose in homogenous matrix form, and $\lambda_a$ denotes the binary values of gripper state. 


\begin{figure*}
  \includegraphics[width=\textwidth]{assets/method.drawio.png}
  % \vspace{-2em}
  \caption{Overview of the proposed method. Our approach first estimates invariant regions in the offline demonstrations of base tasks, as highlighted with \textcolor{darkgreen}{green} masks and \textcolor{darkyellow}{yellow} bounding boxes. Next, these invariant regions are used to train three neural networks to (1) predict invariant regions in new states, (2) find pairwise correspondences between these regions, and (3) find in the demonstration trajectory $\tau$ of some novel task states that are equivalent to a given new state $s_j$. The action pose $T_{j}$ of the new state $s_j$ can be derived by the predicted correspondence, as shown in Equation~\ref{eq:solve}. Our approach generalizes to novel tasks with a single demonstration trajectory and without any fine-tuning.}
  \label{fig:main}
\end{figure*}


\subsection{Task-invariant Regions}
\label{sec:task-inv-space}

We start by introducing the notion of semantic equivalence. Given a task $Task_k\in \mathbf{T}$, two states $s_{i}$ and $s_j$ are said to be semantically equivalent, and denoted as $s_i \equiv s_j$, if the optimal action for solving $Task_k$ in $s_i$ is semantically the same as in $s_j$. 
% \textcolor{red}{For example}
For example, the first semantic action for performing the task `open door' is `reach the door handle', the second semantic action is `grasp the handle', and so on. Therefore, states that describe different scenes with closed doors where the robotic hand has not yet reached a door handle are semantically equivalent, since they all share the optimal action `reach the door handle',
% all share the property that their optimal action is `reach the door handle'.
if the task in question is to open the door. 
Semantic equivalence is loosely defined here and we will define it more precisely in Section \ref{sec:offline-inv-e}.

Next, we consider the following problem. Given an observed transition $(s_i, a_i, s_{i}')$ in a demonstrated trajectory, and a new state $s_j$ such that $s_i \equiv s_j$, how can action %$a_i$ 
pose $T_i$
in state $s_i$ be translated to a new action pose 
$T_j$
% $a_j$ 
to execute in the new state $s_j$? To answer this question, we define the notion of \textbf{invariant region} in the following.

\begin{definition}
    The invariant region of state $s_i$ for $\textrm{Task}_k$ is $\mathcal{I}(s_i|\textrm{Task}_k) = \{ p \in s_i | \forall s_j \in \mathcal{S} \textrm{ s.t. } s_i \equiv s_j, 
\exists q \in s_j: \parallel T^{-1}_{i} p - T^{-1}_{j} q \parallel < \epsilon \}$, where $(T_i,\lambda_i) = \pi^*(s_i|\textrm{Task}_k)$ and $(T_j,\lambda_j) = \pi^*(s_j|\textrm{Task}_k)$. 
% The invariant region of state $s_i$ for a fixed task $\textrm{Task}_k$ is $\mathcal{I}(s_i|\textrm{Task}_k) = \{ p | p \in s_i, \forall s_j \in \mathcal{S} \textrm{ s.t. } s_i \equiv s_j, 
% \exists q \in s_j: \parallel T^{-1}_{i} p - T^{-1}_{j} q \parallel < \epsilon \}$, where $(T_i,\lambda_i) = \pi^*(s_i|\textrm{Task}_k)$ and $(T_j,\lambda_j) = \pi^*(s_j|\textrm{Task}_k)$.\\
% \dhruv{$\mathcal{I}(s_i \vert \text{Task}_k) = \{p \in s_i \vert \exists q \in s_j$, $s_j\equiv s_i$ $ \forall s_j \in \mathcal{S}, \parallel T^{-1}_{i} p - T^{-1}_{j} q \parallel_{2}^{2} < \epsilon \}$}
% \dhruv{In other words, the invariant region is a subset of points $p$ in any state $s_i$ under the task $\text{Task}_k$, where for all semantically equivalent states $s_j \in \mathcal{S}$ under the same task $\text{Task}_k$, there exists a subset of points $q$ in $s_j$ such that the condition given in the above definition is satisfied. 
% Going forward, we will use $\mathcal{I}(s_i)$ interchangeable with $\mathcal{I}(s_i|\text{Task}_k)$ to refer to the invariant region of the state for a fixed task. }
\label{def:inv}
\end{definition}
\noindent $s_i$ is a scene point cloud, and \noindent $\mathcal{I}(s_i|\text{Task}_k)$ is a set of 3D points of $s_i$ whose coordinates remain invariant across all the states in $\mathcal S$ that are semantically equivalent to $s_i$, when viewed in the target end-effector frame $T_{i}$ that is given by the optimal policy $\pi^*$. For example, for the task of picking up a cup, the optimal action is to grasp the cup's handle, regardless of the location, orientation, or style of the cup. The invariant region is likely to be the cup's handle. 
In the following, to simplify the notation, we drop $\textrm{Task}_k$ and simply refer to the invariant region as $\mathcal{I}(s_i)$, while it is implied that $\mathcal{I}(s_i)$ is the invariant region for some fixed task. 
% \dhruv{Given this invariant region $\mathcal{I}(s_i)$, for the new state $s_j$ that is semantically equivalent to $s_i$, its $T_j$ can be infered by finding the correspondence between $\mathcal{I}(s_i)$ and $\mathcal{I}(s_j)$. We define the \textbf{invariance correspondence} in the following.}
Based on these invariant regions, optimal action $T_{j}$ for a new state $s_j$ can be inferred by finding the pairwise correspondence between $\mathcal{I}(s_i)$ and $\mathcal{I}(s_j)$. We define the \textbf{invariance correspondence} in the following.

\begin{definition}
The invariance correspondence between $s_i$ and $s_j$ is $\mathcal{C}(s_i, s_j) = \{(p, q) \in \mathcal{I}(s_i) \times \mathcal{I}(s_j)| q = \argmin_{q\in \mathcal{I}(s_j)} \parallel T^{-1}_{i} p - T^{-1}_{j} q \parallel\}$, where $(T_i,\lambda_i) = \pi^*(s_i|\textrm{Task}_k)$ and $(T_j,\lambda_j) = \pi^*(s_j|\textrm{Task}_k)$. 
\label{def:corr}
\end{definition}

$\mathcal{C}(s_i, s_j)$ is a set of point-level mappings that produce the minimal pairwise distance between the points in $\mathcal{I}(s_i)$ and $\mathcal{I}(s_j)$, when transformed to the target end-effector frames $T_{i}$ and $T_{j}$, respectively. This means that if $\mathcal{C}(s_i, s_j)$ and $T_i$ are both known, then $T_{j}$ can be analytically computed by solving the optimization problem in Equation~\ref{eq:solve} with a standard least-squares algorithm~\citep{huang1986least}, as follows,

% \vspace{-1em}

\begin{equation}
T_j = \arg \min_{T\in \textrm{SE(3)}} \parallel T T^{-1}_{i}  P_{\mathcal{I}(s_i)}  C - P_{\mathcal{I}(s_j)} \parallel,
\label{eq:solve}
\end{equation}

where $P_{\mathcal{I}(s)} \in \mathbb{R}^{4 \times |\mathcal{I}(s)|}$ denotes the points in $\mathcal{I}(s)$, $C \in \{0, 1\}^{|\mathcal{I}(s_i)| \times |\mathcal{I}(s_j)|}$ denotes the binary assignment matrix associated with correspondence $\mathcal{C}(s_i, s_j)$ where $C_{mn} = 1$ if and only if $(p_m, q_n) \in \mathcal{C}(s_i, s_j)$. 

While Equation~\ref{eq:solve} provides a solution to computing action $T_{j}$, mining a set of pairs of equivalent states $(s_i, s_j)$ from the offline demonstrations, and finding invariant regions $\mathcal{I}(s_i)$ remain unsolved. We address this in the following section.

\subsection{Offline Invariant Region Estimation}
\label{sec:offline-inv-e}

We consider the problem of estimating invariant 
% 3D 
regions $\mathcal{I}(s_i)$ for all the states $s_i$ that appear in the dataset $\mathcal{D}_{base}$ of offline demonstrations. One classical way to address this issue is to manually select and label pairs of semantically equivalent states for every task through annotation~\citep{gu2018ava}, and solve $\mathcal{I}(s_i)$ as in Definition~\ref{def:inv}. %Then, $\mathcal{I}(s_i)$ can be solved through optimization with constraints $\parallel T^{-1}_{a_i} p - T^{-1}_{a_j} q \parallel < \epsilon, \forall s_i \equiv s_j$. 
However, manual annotation is labor-intensive. Instead, we propose an unsupervised empirical approach to directly estimate  $\mathcal{I}(s_i)$. 
Then, for each state $s_i$,  
% 6D 
action pose $T_j$ is computed for each other state $s_j$ in 
$\mathcal{D}_{base}$ using Equation~\ref{eq:solve}, under the hypothesis that $s_i \equiv s_j$. 
Since the ground-truth value of $T_{j}$ is available in $\mathcal{D}_{base}$, we automatically label $s_i$ as semantically equivalent to $s_j$ if the 
% average
estimation error of $T_{j}$ is smaller than a pre-defined threshold. The same threshold is used for all the tasks. 

To estimate $\mathcal{I}(s_i)$, we first obtain a set of candidate state pairs $\mathcal{D}_{align}$ through a naive trajectory alignment procedure, which matches time-steps from different trajectories of the same task in $\mathcal{D}_{base}$ based solely on the length of each trajectory and without considering the values of the actions or the states in the trajectory. We detail this simple pre-processing procedure in Section~\ref{sec:impl-detail}. The expected displacement $\Delta_{s_i}(p)$ of a point $p \in s_i$ in the target end-effector frame is defined as follows,
%\vspace{-1.5em}
\begin{equation}
\Delta_{s_i}(p) = \mathbb{E}_{(s_i, s_j) \in \mathcal{D}_{align}} \left[\min_{q \in s_j} \parallel T^{-1}_{i} p - T^{-1}_{j} q \parallel \right]
\label{eq:delta}
\end{equation}

% where $T_i$ and $T_j$ are respectively the 6D poses of the end-effector in states $s_i$ and $s_j$ in the demonstrations.  
%
where  $T_i$ and $T_j$ are respectively the target end-effector poses of states $s_i$ and $s_j$ in the recorded demonstrations.
Then, we cluster the points in state $s_i$ into $N$ segments $\{c_{i,n}\}_{n=1}^N$, where each segment $c_{i,n} \subseteq s_i$ is a set of 3D points.
We define the invariant region $\mathcal{I}(s_i)$ for the given task as the segment with the minimal average displacement,

%\vspace{-1em}
\begin{equation}
\mathcal{I}(s_i) = \arg\min_{c_{i, n}} \mathbb{E}_{p \in c_{i, n}} [\Delta_{s_i}(p)].
\label{eq:segment}
\end{equation}
To determine if $s_i \equiv s_j$, we align $\mathcal{I}(s_i)$ to $\mathcal{I}(s_j)$ through point-set registration, and compute $err(s_i, s_j)$, the alignment error of the target end-effector pose,
\begin{equation}
\begin{gathered}
T_{\mathcal{I}(s_i) \rightarrow \mathcal{I}(s_j)} = \text{Align}\left(\mathcal{I}(s_i), \mathcal{I}(s_j)\right) \\
err(s_i, s_j) = \parallel T_{\mathcal{I}(s_i) \rightarrow \mathcal{I}(s_j)} T_{i}  - T_{j} \parallel
\end{gathered}
\label{eq:C-reg}
\end{equation}
where $T_{\mathcal{I}(s_i) \rightarrow \mathcal{I}(s_j)} \in \mathbb{R}^{4\times 4}$ denotes the alignment transformation matrix, and the iterative closest point method~\citep{besl1992method} is used for alignment. We define $s_i \equiv s_j$ if $err(s_i, s_j) < \gamma$, where $\gamma$ is a global hyper-parameter. In Equation~\ref{eq:dpair}, we define $D_{pair}$ as the set of the semantically equivalent state pairs in $D_{align}$.
\begin{equation}
D_{pair}=\{(s_i, s_j) | (s_i, s_j) \in \mathcal{D}_{align}, err(s_i, s_j) < \gamma \}
\label{eq:dpair}
\end{equation}

In this section, we have shown how to estimate $\mathcal{I}(s_i)$ and to discover semantically equivalent states in the offline dataset $\mathcal{D}_{base}$. In Section~\ref{sec:algo}, we show how to predict, simply through learning, invariant regions of the states that appear in one-shot demonstrations of novel tasks, and during testing in new scenes.



\subsection{Algorithm}
\label{sec:algo}


% \begin{minipage}{\columnwidth}
\begin{algorithm}%[H]
   \caption{IMOP Training}
   \label{alg:train}
\begin{algorithmic}[1]
   \STATE {\bfseries Input:} Dataset $\mathcal{D}_{base}$ of unannotated demonstrations; 
\STATE Initialize neural network weights $\theta$ with random values
   \STATE Use Equation~\ref{eq:dpair} to automatically extract a set of semantically equivalent state pairs $\mathcal{D}_{pair}$ from $\mathcal{D}_{base}$
   \REPEAT
   \STATE Sample a state pair $(s_i, s_j)$ from $\mathcal{D}_{pair}$

    \STATE Retrieve $(s_i, a_i, s'_{i})$ and $(s_j, a_j, s'_{j})$ from $\mathcal{D}_{base}$
    \STATE Randomly sample a state $s_k$ from $\mathcal{D}_{base}$

   \STATE $\widehat{\mathbf{P}}[p \in \mathcal{I}(s_i)] \leftarrow f_\mathcal{I}(s_i, s'_{i}; \theta)$
   \STATE $I_{s_i} \leftarrow \mathbb{I}[p \in \mathcal{I}(s_i)]$
   
   \STATE $\widehat{\mathbf{P}}[(p, q) \in \mathcal{C}(s_i, s_j)] \leftarrow f_\mathcal{C}(s_i, s_j, I_{s_i}; \theta)$

   \STATE Compute $\mathcal{C}(s_i, s_j)$ with $\mathcal{I}(s_i), \mathcal{I}(s_j)$ as in Def.~\ref{def:corr}

   \STATE $\widehat{\mathbf{P}}[s_i \equiv s_j] \leftarrow f_\mathcal{S}(s_i, s_j;\theta)$
   \STATE $\widehat{\mathbf{P}}[s_i \equiv s_k] \leftarrow f_\mathcal{S}(s_i, s_k;\theta)$

   \STATE \scalebox{1}{$\mathcal{L}_{\mathcal{S}} \leftarrow \mathcal{L}_{\text{focal}}\big(\widehat{\mathbf{P}}[s_i \equiv s_k] , 0\big) + \mathcal{L}_{\text{focal}}\big(\widehat{\mathbf{P}}[s_i \equiv s_j], 1\big)$}
    
   
   \STATE $\mathcal{L}_\mathcal{I} \leftarrow \mathcal{L}_{\text{focal}}\big(\widehat{\mathbf{P}}[p \in \mathcal{I}(s_i)], \mathcal{I}(s_i)\big)$
   
   \STATE $\mathcal{L}_\mathcal{C} \leftarrow \mathcal{L}_{\text{focal}}\big(\widehat{\mathbf{P}}[(p, q) \in \mathcal{C}(s_i, s_j)], \mathcal{C}(s_i, s_j)\big)$
   
   \STATE Update $\theta$ with backpropagation from $\mathcal{L}_\mathcal{S} + \mathcal{L}_\mathcal{I} + \mathcal{L}_\mathcal{C}$
   \UNTIL{converged}
\end{algorithmic}
\end{algorithm}


We design a new neural network that predicts the invariant region $\mathcal{I}(s_i)$ given an observed transition $(s_i, a_i, s'_{i})$ in the one-shot online demonstration, and predicts $\mathcal{C}(s_i, s_j)$ for a new state $s_j$ by matching $s_i$ and $s_j$. In doing so, we present the \textbf{I}nvariance \textbf{M}atching \textbf{O}ne-shot \textbf{P}olicy Learning (IMOP) algorithm.  We summarize the training and evaluation of IMOP in Algorithms~\ref{alg:train} and~\ref{alg:eval}. The overall architecture is illustrated in Figure~\ref{fig:main}. We detail this procedure in the following. 

To predict $\mathcal{I}(s_i)$, we design the invariance estimator function $f_{\mathcal{I}}: \mathcal{S}\times \mathcal{S}\times \Theta \mapsto [0, 1]^{|s|}$, where $\Theta$ denotes the network parameter space, and $|s|$ denotes the number of points in a state. $f_{\mathcal{I}}$ takes two consecutive states $s_i$ and $s'_{i}$ as input and returns a pointwise probability map $\widehat{\mathbf{P}}[p \in \mathcal{I}(s_i)]$, as indicated in line 8 of Algorithm~\ref{alg:train}. The invariant region is obtained by thresholding this probability map and turning it to a pointwise binary mask as done in line 9 of Algorithm~\ref{alg:eval}. $f_{\mathcal{I}}$ is trained by focal loss~\citep{lin2017focal} with $\mathcal{I}(s_i)$ in the offline data as ground-truth labels, as done in line 15 of Algorithm~\ref{alg:train}.


To predict the pairwise correspondence map $\mathcal{C}(s_i, s_j)$, and derive $T_{j}$ subsequently, we design the invariance matcher function $f_\mathcal{C}: \mathcal{S} \times \mathcal{S} \times \{0, 1\}^{|s|} \times \Theta \mapsto [0, 1]^{|\mathcal{I}(s_i)| \times |s_j|}$, where $|\mathcal{I}(s_i)|, |s_i|$ and $|s_j|$ denote the number of points in $\mathcal{I}(s_i)$, $s_i$, and $s_j$, respectively.
$f_\mathcal{C}$ takes $s_i$, $s_j$ and $I_{s_i}$ as input and predicts a pairwise probability $\widehat{\mathbf{P}}[(p, q) \in \mathcal{C}(s_i, s_j)]$ as in line 10 of Algorithm~\ref{alg:train}, where $I_{s_i}$ denotes the binary mask representation of $\mathcal{I}(s_i)$. $f_{\mathcal{C}}$ is trained by focal loss with $\mathcal{C}(s_i, s_j)$ as labels, where $\mathcal{C}(s_i, s_j)$ is computed from $\mathcal{I}(s_i)$ and $\mathcal{I}(s_j)$ in the offline data, as in lines 11 and 16 of Algorithm~\ref{alg:train}.
The output of $f_\mathcal{C}$ is a soft assignment matrix $C \in [0, 1]^{|\mathcal{I}(s_i)| \times |s_j|}$. The target end-effector pose $T_j$ of state $s_j$ can be obtained by substituting $\mathcal{I}(s_j)$  with $s_j$ in Equation~\ref{eq:solve}, where $P_{I_{s_i}} \in \mathbb{R}^{4\times |\mathcal{I}(s_i)|}$ and $P_{s_j} \in \mathbb{R}^{4\times |s_j|}$ respectively denote the points of $\mathcal{I}(s_i)$ and $s_j$ in a matrix form, as in lines 9 and 10 of Algorithm~\ref{alg:eval}. 




To determine whether $s_i \equiv s_j$, we design the state matcher function $f_\mathcal{S}:  \mathcal{S} \times \mathcal{S} \times \Theta \mapsto [0, 1]$. $f_\mathcal{S}$ takes $s_i$ and $s_j$ as input and returns the probability $\widehat{\mathbf{P}}[s_i \equiv s_j]$ as in line 12 of Algorithm~\ref{alg:train}. $f_{\mathcal{S}}$ is trained by focal loss with state pairs in $\mathcal{D}_{pair}$ as pseudo ground-truth positive samples and random state pairs as negative ones, as in line 14 of Algorithm~\ref{alg:train}. 

During inference in a new scene, and given a one-shot demonstration $\tau$ of some novel task, $(s_i, a_i, s_i') \in \tau$ is chosen by the largest $\widehat{\mathbf{P}}[s_i \equiv s_j]$ for each query state $s_j$, as in lines 4-7 of Algorithm~\ref{alg:eval}. 
The gripper state $\lambda_i$ of $s_i$ (the binary parts of the action that indicate whether the gripper is closed or open, and whether collisions are allowed or not) is copied directly as the prediction for $\lambda_j$ in the new state $s_j$, as in line 11 of Algorithm~\ref{alg:eval}. A test trial ends when the demonstration trajectory $\tau$ has been consumed, as in line 14 of Algorithm~\ref{alg:eval}.


% \end{minipage}
% \begin{minipage}{\columnwidth}
\begin{algorithm}%[H]
   \caption{IMOP Inference}
   \label{alg:eval}
\begin{algorithmic}[1]
   \STATE {\bfseries Input:} Invariance estimator $f_{\mathcal{I}}$; Invariance matcher $f_\mathcal{C}$; State matcher $f_{\mathcal{S}}$; Trained network parameters $\theta$; Novel task one-shot demonstration trajectory $\tau$; Initial state $s_j$
    \STATE $t \leftarrow 0$
    \REPEAT 
   \FORALL{$(s_k, a_k, s'_{k}) \in \tau$}
   \STATE $\widehat{\mathbf{P}}[s_k \equiv s_j] \leftarrow f_\mathcal{S}(s_k, s_j;\theta)$
   \ENDFOR
   \STATE $i \leftarrow \argmax_{k} \widehat{\mathbf{P}}[s_k \equiv s_j]$
   \STATE $I_{s_i} \leftarrow \mathbb{I}[f_\mathcal{I}(s_i, s'_{i}; \theta) > 0.5]$
   \STATE $C \leftarrow f_\mathcal{C}(s_i, s_j, I_{s_i};\theta)$
   \STATE Solve $T_j = \argmin_{T\in \textrm{SE(3)}} \parallel T T_i^{-1} P_{I_{s_i}} C - P_{s_j} \parallel$
   \STATE $a_j \leftarrow (T_j, \lambda_{i})$
   \STATE Execute $a_j$ and sample the next state $s'_j$ from $\mathbf{P}(. | s_j, a_j)$
   \STATE $t \leftarrow t + 1$, $s_j \leftarrow s'_j$
   \UNTIL{$t > |\tau|$}
\end{algorithmic}
\end{algorithm}
% \end{minipage}




\subsection{Implementation Details}
\label{sec:impl-detail}


We build $f_\mathcal{I}$, $f_\mathcal{S}$, and $f_\mathcal{C}$ using graph neural networks. Figure~\ref{fig:network} illustrates the different neural network architectures used. First, we extract point-level features using a point transformer network~\citep{zhao2021point} over the KNN graphs of the individual point clouds $s_i, s_i'$ and $s_j$. These features are extracted at two resolutions represented as coarse and fine points in Figure~\ref{fig:network}. 
Next, we use the point transformers on KNN graphs built between different point clouds, for example, the KNN graphs between $s_i$ and $s_i'$ are constructed to encourage the network to learn cross-scene information. 
Notably, for $f_\mathcal{I}$ and $f_\mathcal{S}$, the KNN graphs are built on coarse points to encourage interactions over larger spaces. Figure~\ref{fig:knn-points} illustrates the structure of the KNN graphs, and coarse and fine points. Finally, the output of $f_\mathcal{I}$ and $f_\mathcal{S}$ are derived by applying a linear layer upon the point features. For $f_\mathcal{C}$, a cross attention layer is used between the point features of $\mathcal{I}(s_i)$ and $s_j$ to produce the probability matrix. 

Point transformer applies attention between the adjacent nodes of a graph and is more efficient than a traditional transformer for graph data because the degree of a graph is usually much smaller than the total number of nodes~\citep{lu2022transformers}. The original point transformer only supports self-attention on graphs built from a single point cloud~\citep{zhao2021point}. We extend it to support cross-attention on KNN graphs built from different point clouds. Our point transformer network is based on the PTv2~\citep{wu2022point} implemented in Pointcept~\citep{pointcept2023}, and PyTorch3D~\citep{ravi2020pytorch3d}. We use the soft Procrustes operator from Lepard~\citep{li2022lepard} to solve the least-squares problem in line 10 of Algorithm~\ref{alg:eval}. 




For the offline invariant region estimation in Section~\ref{sec:offline-inv-e}, we use HDBSCAN clustering~\citep{mcinnes2017hdbscan} and segmentation masks provided by RLBench~\citep{james2020rlbench} to create segments $\{c_{s_i,n}\}_{n=1}^N$ and remove the segments on the robot. Remark that the segmentation masks are only used for the offline estimation of $\mathcal{I}(s_i)$.
For the trajectory alignment, we denote $\tau_{k_m} = \{(s_{k_m,j}, a_{k_m,j}, s_{k_m,j+1})\}_{j=1}^{|\tau_{k_m}|}, m \in [H_k], k \in [K]$ as a trajectory for task $k$ in $\mathcal{D}_{base}$, where $H_k$ denotes the number of trajectories for task $k$, and $K$ denotes the number of tasks.
% We skip the task notation $k$ for simplicity.
As in Equation~\ref{eq:pair0}, $\tau_{k_m}$ and $\tau_{k_n}$ are aligned with indexes $j_1 = \round{{j \cdot |\tau_{k_m}}|/M}$ and $j_2 = \round{{j \cdot |\tau_{k_n}}|/M}$, where $M = \max(|\tau_{k_m}|, |\tau_{k_n}|)$ and $j\in[M]$.
% by which $(s_{k_m,j_1}, s_{k_n, j_2})$ are matched
For example, if the lengths of $\tau_{k_m}$ and $\tau_{k_n}$ are 2 and 4, then $s_{k_m,1}$ is matched with $s_{k_n,1}$ and $s_{k_n,2}$, and $s_{k_m,2}$ is matched with $s_{k_n,3}$ and $s_{k_n,4}$.


% For the trajectory alignment, we denote $\tau_k = \{(s_{k,i}, a_{k,i}, s_{k,i+1})\}_{i=1}^{H_{\tau_k}}, k \in [K]$ as a trajectory for task $k$ in $\mathcal{D}_{base}$, where $K$ and $H_{\tau_k}$ denote the number and lengths of trajectories. We skip the task notation $k$ for simplicity.
% As in Equation~\ref{eq:pair0}, $\tau_1$ and $\tau_2$ are aligned with indexes $i_1 = \round{{i \cdot H_{\tau_{k_1}}}/{H_{max}}}$ and $i_2 = \round{{i \cdot H_{\tau_{k_2}}}/{H_{max}}}$, by which $(s_{k_1,i_1}, s_{k_2, i_2})$ are matched. 

% \vspace{-1em}

\begin{nalign}
\mathcal{D}_{align} = \{(s_{k_m,j_1}, s_{k_n, j_2}) | j_1 = \round{{j \cdot |\tau_{k_m}|}/{M}}, \\ 
j_2 =  \round{{j \cdot |\tau_{k_n}|}/{M}}, 
\\ j \in [M], M = \max(|\tau_{k_m}|, |\tau_{k_n}|), \\
\forall m, n \in [H_k], m \neq n, \\
\forall k \in [K] \}
\label{eq:pair0}
\end{nalign}


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{assets/arch.drawio.png}
    \caption{Network architectures of $f_\mathcal{I}$, $f_\mathcal{S}$, and $f_\mathcal{C}$.}
    \label{fig:network}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{assets/arch_additional.drawio.png}
    \caption{Illustrations of KNN graphs used in the neural networks, and coarse and fine points from Figure~\ref{fig:network}. KNN graphs are built by connecting each point to the nearest $k$ points in Euclidean distances. KNN graphs between $s_i$ and $s_j$ include both the connections from $s_i$ to $s_j$ and $s_j$ to $s_i$. 
    We only visualize the connections of two points, within $s_i$ and from $s_i$ to $s_j$, for clarity.
    Each point within the coarse and fine points includes a spatial coordinate and a feature vector. Coarse points have a higher dimension of feature vectors, but fewer points and lower resolution, and vice versa for fine points.
    Only the spatial coordinates are used in constructing the KNN graphs.}
    \label{fig:knn-points}
\end{figure}


==> modules.backup/6.experiment.tex <==

\begin{table*}[h]\centering
\caption{Base Task Performance on RLBench. We report the success rate for each task, and measure the average success rate and rank across all tasks. IMOP has the best overall success rate and rank. The success rate of IMOP is measured with an average of 5 runs. The success rates of baselines are reported from respective papers.}\label{tab:base}
% \vspace{-1em}
\footnotesize
% \resizebox{\linewidth}{!}{
\begin{tabular}{lcccccccccc}\toprule
\multirow{2}{*}{Method} &Avg. &Avg. &Close &Drag &Insert &Meat off &Open &Place &Place &Push \\ %\cmidrule{2-11}
&Success &Rank &Jar &Stick &Peg &Grill &Drawer &Cups &Wine &Buttons \\\midrule
C2F-ARM~\citep{james2022coarse} &20.1 &4.9 &24 &24 &4 &20 &20 &0 &8 &72 \\
PerAct~\citep{shridhar2023perceiver} &49.4 &3.6 &55.2 &89.6 &5.6 &70.4 &88 &2.4 &44.8 &92.8 \\
RVT~\citep{goyal2023rvt} &62.9 &2.3 &52 &\textbf{99.2} &11.2 &88 &71.2 &4 &91 &\textbf{100} \\
Act3D~\citep{gervet2023act3d} &65.1 &2.2 &\textbf{92} &92 &\textbf{27} &\textbf{94} &93 &3 &80 &99 \\
IMOP (Ours) &\textbf{69.6} &\textbf{1.9} &38.8 &98.4 &12.0 &92.0 &\textbf{100.0} &\textbf{53.2} &\textbf{96.0} &94.4 \\\midrule
&Put in &Put in &Put in &Screw &Slide &Sort &Stack &Stack &Sweep to &Turn \\
&Cupboard &Drawer &Safe & Bulb & Block & Shape & Blocks & Cups & Dustpan & Tap \\\midrule
C2F-ARM~\citep{james2022coarse} &0 &4 &12 &8 &16 &8 &0 &0 &0 &68 \\
PerAct~\citep{shridhar2023perceiver} &28 &51.2 &84 &17.6 &74 &16.8 &26.4 &2.4 &52 &88 \\
RVT~\citep{goyal2023rvt} &49.6 &88.0 &91.2 &48 &81.6 &36 &28.8 &26.4 &72 &93.6 \\
Act3D~\citep{gervet2023act3d} &\textbf{51} &90 &95 &47 &\textbf{93} &8 &12 &9 &92 &\textbf{94} \\
IMOP (Ours) &46.8 &\textbf{100.0} &\textbf{96.0} &\textbf{81.6} &58.4 &\textbf{37.2} &\textbf{40.0} &\textbf{57.2} &\textbf{100.0} &50.8 \\
\bottomrule
\end{tabular}
% }
\end{table*}

\section{Experiments}
\label{sec:experiment}



We evaluate \textbf{IMOP} on the visual robotic manipulation tasks from RLBench~\citep{james2020rlbench}, a standard benchmark used in multi-task learning~\citep{james2022q}. We first train and evaluate our algorithm on the standard 18 RLBench tasks, and then measure its one-shot generalization ability on 22 novel tasks from 9 categories~\citep{guhur2023instruction}.
Further, we evaluate our method in real-robot experiments through one-shot sim-to-real transfer. 
Specifically, we aim to answer the following questions:

\begin{itemize}
    \item Can IMOP achieve high success rates on base tasks? 
    \item Can IMOP generalize to novel tasks given a single demonstration without tuning? 
    \item Can IMOP generalize to objects with large shape variations? 
    \item Can IMOP estimate meaningful invariant regions from demonstrations of novel tasks?
    
    \item Can IMOP be trained in simulation and transferred to solve real-robot manipulation tasks?
\end{itemize}

\textbf{Environment.} Following the convention~\citep{goyal2023rvt}, we record $128\times128$ RGB-D images from the front, left/right-shoulders, and wrist cameras. During training, we use 100 recorded trajectories per base task. % without requiring access to online simulators. 
RLBench contains various task categories, such as pick-and-place, tool use, high-precision operations, screwing, tasks with visual occlusion, and long-term manipulation. We choose 22 novel tasks that have different object setups and task goals from the base ones, according to the task categorization of Hiveformer~\citep{guhur2023instruction}. 
For each novel task, only a single successful trajectory is provided, as a one-shot demonstration.
Each task is evaluated on 25 independent trials, and we report the average success rate. RLBench generates different object layouts and orientations in different trials of the same task. For the base tasks, we use the same test scenes as the ones in~\citep{james2022q}. For novel tasks, we generate 25 test scenes for each task. Figure~\ref{fig:rlbench} illustrates the task,  and object-level generalizations of IMOP within the RLBench environment.
Further details are provided in the supplementary material.




\subsection{Performance Comparison on Base Tasks}
\label{sec:exp-base}


\textbf{Baselines.} To evaluate the performance of IMOP on base tasks, we test policies learned from offline demonstrations without the one-shot demonstrations. Specifically, we consider C2F-ARM~\citep{james2022coarse}, PerAct~\citep{shridhar2023perceiver}, RVT~\citep{goyal2023rvt}, and Act3D~\citep{gervet2023act3d}. C2F-ARM and PerAct learn separate policies for each task. Similar to our IMOP, RVT and Act3D learn a single multi-task policy. 

\textbf{Results.}  Table~\ref{tab:base} compares the success rates of IMOP and other baselines on the base tasks. C2F-ARM and PerAct use 3D voxel representation. RVT renders point clouds to virtual images. Similar to IMOP, Act3D uses raw point clouds as states. Overall, IMOP outperforms all baselines when the best rank and success rate are averaged across all tasks ($+4.5\%$ average success rate). IMOP has the highest rank on 10 out of 18 tasks. Remarkably, IMOP achieves a success rate of $53.2\%$ on the ``place cups" task while the existing works only reach a rate of $2\%$ to $4\%$. Moreover, not only it outperforms existing techniques, IMOP also generalizes to novel tasks, while the baselines can only be used on the tasks they were trained on.   


\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{assets/inv.drawio.png}
    \caption{Visualization of invariant regions $\mathcal{I}(s_i)$ as estimated by $f_\mathcal{I}$ on selected base and novel tasks. The invariant regions on $s_i$ are highlighted with \textcolor{darkgreen}{green} masks and \textcolor{darkyellow}{yellow} bounding boxes. The end-effector position is marked with \textcolor{darkred}{red} dot. $\mathcal{I}(s_i)$ generally covers the target object of the action that is applied by the robot to transition from state $s_i$ to next state $s'_{i}$. For example, the invariant region of `turn the lamp on' covers the `lamp switch' area. The invariant region of `pull the rope straight' covers one side of the rope and the rope target. It is worth noting that the invariance estimator $f_\mathcal{I}$ only takes point cloud as input and has no access to segmentation masks. }
    \label{fig:inv}
\end{figure*}

\subsection{Generalization to Novel Tasks}
\label{sec:exp-novel}

\begin{table*}[h]\centering
\caption{Novel Task Performance on RLBench. We report the success rate for each task, and measure the average success rate and rank across all tasks. IMOP has the best overall success rate and rank. Both RVT+FT and RVT+HDT require fine-tuning but IMOP does not. Directly using RVT without fine-tuning results in an average success rate of 0. We do not include this in the table. All success rates are measured with an average of 5 runs. }\label{tab:novel}
% \vspace{-1em}
% \scriptsize     
\footnotesize
% \resizebox{\linewidth}{!}{
\begin{tabular}{lcccccccccccc}\toprule
\multirow{2}{*}{Method} &Avg. &Avg. &Ball in &Rubbish &Scoop &Place &Hit &Block &Slide &Phone &Open &Close \\
&Success &Rank &Hoop &in Bin &Spatula & Hanger & Ball & Pyramid & Place &on Base & Box & Lid \\\midrule
RVT+FT &29.8 &2 &42.4 &50 &7.2 &4 &1.6 &0 &0 &20.4 &\textbf{28} &\textbf{100} \\
RVT+HDT &26.9 &2.4 &\textbf{87.6} &40.4 &0 &0 &0 &0 &0 &0 &24.8 &91.2 \\
IMOP (Ours) &\textbf{41.3} &\textbf{1.5} &76.0 &\textbf{94.8} &\textbf{52.0} &\textbf{25.2} &\textbf{32.0} &\textbf{5.2} &\textbf{6.8} &\textbf{22.8} &8.0 &69.6 \\\midrule
&Lid off &Lamp &Beat &Remove &Play &Knife on &Straighten &Change &Open &Open &Money  &Close \\
&Pan & On & Buzz &Cups &Jenga & Board &Rope & Clock &Bottle &Door &out Safe &Microwave \\\midrule
RVT+FT &78.8 &65.2 &19.2 &4 &40.8 &14 &0 &10.4 &34.4 &\textbf{68} &22.4 &44 \\
RVT+HDT &80.4 &\textbf{72} &16.4 &0 &27.6 &8 &0 &\textbf{36} &23.2 &12 &12 &\textbf{59.6} \\
IMOP (Ours) &\textbf{100.0} &12.0 &\textbf{20.0} &\textbf{36.0} &\textbf{100.0} &\textbf{20.0} &\textbf{17.2} &24.0 &\textbf{81.2} &41.6 &\textbf{42.8} &21.2 \\
\bottomrule
\end{tabular}
% }
\end{table*}


\textbf{Baselines.} To assess the one-shot ability of IMOP, and since there is no existing one-shot learning method in the literature that was evaluated in RLBench, we extend the state-of-the-art technique RVT into two baselines, called RVT+FT and RVT+HDT, that can be used for one-shot learning. Specifically, since fine-tuning is the most common strategy for transferring models to new domains~\citep{yu2022survey}, we fine-tune RVT models pretrained on the base tasks with demonstrations of novel tasks and denote this baseline as RVT+FT. HDT~\citep{xu2023hyper} is a recent work that achieves one-shot policy generalization by training additional adaptation layers for new tasks while freezing original parameters. We implement the HDT adaptation layers in RVT and denote this baseline model as RVT+HDT. RVT and Act3D are both the most recent methods for learning multi-task robot control policies, and have similar performances, as shown in Table~\ref{tab:base}. We choose RVT over Act3D because the pretrained model of the latter is not yet available. For both RVT+FT and RVT+HDT, we train the respective network parameters with the one-shot demonstrations of novel tasks until convergence and adopt the sampling and 3D perturbation augmentation strategy from RVT and PerAct. 
% During testing, one demonstration trajectory for each novel task is provided. 



\textbf{Results.} Table~\ref{tab:novel} compares the  success rates of IMOP, RVT+FT, and RVT+HDT on novel task. IMOP outperforms all baselines with the best rank and success rate averaged across all tasks ($+11.5\%$ over RVT+FT). IMOP has the best rank on 15 out of 22 tasks. Despite using the simple fine-tuning strategy, RVT+FT performs better than RVT+HDT on novel tasks. However, we observe the catastrophic forgetting phenomenon~\citep{kirkpatrick2017overcoming} in RVT+FT, whose average success rate on base tasks plummets to $4.6\%$ from $62.9\%$ after fine-tuning on novel tasks. RVT-HDT maintains the base task performance by freezing the original parameters but at the cost of having more parameters in the adaptation layers. Parameter sizes are compared in Table~\ref{tab:params}. 



\begin{figure*}
\hspace{-1em}
  \includegraphics[width=\linewidth]{assets/sim2real.drawio.png}
  % \vspace{-2em}
  \caption{Real-robot manipulation examples of IMOP via one-shot sim-to-real transfer. The invariance correspondences between the demonstration and test scenes are shown in \textcolor{darkred}{red} lines. The invariant regions closely overlap the next object to be picked up, and the target object or container to be placed. We observe that the one-shot generalization capacity of IMOP, trained with simulation data, enables the sim-to-real transfer using a single real-world demonstration without any re-training.}
  
  \label{fig:real-robot-exp}
\end{figure*}


\begin{table}[!htp]\centering
\caption{Network parameters size comparison between IMOP and one-shot baselines.}\label{tab:params}
\begin{tabular}{lcccc}\toprule
&\multicolumn{2}{c}{Success Rate (\%)} &\multirow{2}{*}{Params Size} \\
Method &Base &Novel & \\\midrule
RVT+FT &4.7 &29.8 &104M \\
RVT+HDT &62.9 &26.9 &131M \\
Ours &69.6 &41.3 &80.8M \\
\bottomrule
\end{tabular}
\end{table}

Compared to the baselines, IMOP generalizes to novel tasks by matching invariant regions between the one-shot demonstration and the states encountered during testing, without further training. Therefore, IMOP does not suffer from catastrophic forgetting or increased size of the parameters. Remarkably, both RVT+FT and RVT+HDT completely fail on certain tasks, \textit{e.g.}, ``block pyramid", ``slide place", and ``straighten rope", while IMOP still delivers a non-trivial performance on these tasks. Both ``block pyramid" and ``slide place" are categorized as long-horizon tasks and require over 30 and 10 macro-steps, respectively, to finish~\citep{guhur2023instruction}. The ``straighten rope" task requires operations on ropes, which are drastically different from the objects in the base tasks. This further indicates the limitation of the existing one-shot policy generalization strategies and the advantage of our proposed invariance matching-based policy. Figure~\ref{fig:inv} visualizes invariant regions on selected base and novel tasks. It can be seen that the invariant regions generally cover the target objects of the robot's actions. Additional visualizations are provided in the supplementary material.


\textbf{Analysis of underperformed tasks.} Despite the overall superiority of IMOP, the performance on specific tasks is still worth discussing. As in Table~\ref{tab:novel}, IMOP exhibits a lower success rate on `open box', `close microwave', and `close lid' compared to RVT+FT and RVT+HDT. These tasks involve manipulating flat surfaces, such as lids and box covers, as shown by the invariant region of `open box' visualized in Figure~\ref{fig:inv}. 
The challenge arises from the potential ambiguity in identifying invariant regions or correspondences on flat surfaces lacking rich geometric features. 
IMOP also performs worse than the baselines on the `lamp on' task, as you can see in the first two columns of Figure~\ref{fig:inv}. Although the invariant region estimation for this task is good, the area of the switch is small and hence, the invariance correspondence is sparse compared to the whole scene, which leads to unstable solutions of the least-square problem in Equation~\ref{eq:solve}. The success rate of IMOP on long-term tasks, \textit{i.e.}, `block pyramid' and `slide place', outperforms the baseline methods but still has a large room for improvement. The IMOP mechanism of matching new states in test scenes to demonstrations is simple yet lacks the failure recovery ability because the demonstrations only contain successful trajectories. 




\subsection{Generalization to Large Shape Variations}
\label{sec:exp-beyond-demo}


\begin{figure}
    \centering
    \captionsetup[subfigure]{justification=centering,labelformat=empty}
    \subfloat[`Spam' $\rightarrow$ `Crackers']{\includegraphics[width=0.49\linewidth]{assets/cross_object/7-15.png}}\hfill
    \subfloat[][`Mustard' $\rightarrow$ `Sugar box']{\includegraphics[width=0.49\linewidth]{assets/cross_object/30-35.png}}

    \vspace{-0.8em}

    \subfloat[`Coffee jar' $\rightarrow$ `Soup can']{\includegraphics[width=0.49\linewidth]{assets/cross_object/21-10.png}}\hfill
    \subfloat[][`Choco jello' $\rightarrow$ `Tuna can']{\includegraphics[width=0.49\linewidth]{assets/cross_object/28-27.png}}
    \caption{Visualization of invariance correspondence between different objects for the picking action. `Spam' $\rightarrow$ `Crackers' denotes using `Spam' as the demonstration to correspond to `Crackers' during testing.  
    Despite large shape variations, IMOP is able to estimate correspondences that effectively transfer actions, as shown by the success rate in Figure~\ref{fig:cross-object}.}
    \label{fig:corr-vis}
\end{figure}


\textbf{Setup.} Previous experiments evaluate the one-shot generalization ability of IMOP on novel tasks with one demonstration trajectory for each task. Even though there are large 
 variations in object shapes and categories between base and novel tasks, the variations within each novel task are limited.
%%%%%%%%%
For example, the novel task `put the knife on the chopping board' includes objects such as a knife, knife holder, and chopping board. 
None of these objects are seen during training and they are placed randomly at each trial and sometimes with color variations, but the object categories and shapes remain unchanged among various trials, as illustrated in Figure~\ref{fig:rlbench}. 
We are interested in whether IMOP can generalize to objects with large shape variations. 
To study this, we evaluate IMOP on objects different from those in demonstrations, which naturally have different shapes. Specifically, we consider a pick-and-place setting where the objective is to pick groceries and place them into a cupboard. 
The demonstration is given on a certain object, but picking and placing a different object is required during testing.
To simplify our study, we assume the access of the segmentation mask of the required object during testing.
Therefore, the correspondence between different objects can be obtained by masking out other regions.
To avoid memorization, we remove the corresponding state pairs from the training data. 



\begin{figure}
  \includegraphics[width=\linewidth]{assets/cross_object.pdf}
  % \vspace{-2em}
  \caption{Success rate of pick-and-place task using different objects with large shape variations as demonstrations. For example, the entry at the top-right corner, \textit{i.e.}, `berry-jello, tuna', denotes the success rate is 30\% at picking and placing `tuna can' while using `berry-jello box' as the demonstration.}
  \label{fig:cross-object}
\end{figure}


\textbf{Result.} Figure~\ref{fig:cross-object} shows the success rate of pick-and-place with demonstrations on different objects. For example, the entry `mustard, coffee' represents the success rate of 
picking and placing a coffee jar with a demonstration on a mustard bottle.
There are 9 objects in total, and all success rates are measured on an average of 10 trials. It can be seen that IMOP performs competitively when a different object is used as a demonstration, except in some cases of the mustard bottle whose shape is drastically different than others. Using berry-jello and choco-jello as demonstrations delivers the same or even better results on many objects during testing, \textit{e.g.}, soup, spam, sugar, and tuna. These two jello boxes are the smallest objects in this setup. 



Figure~\ref{fig:corr-vis} visualizes the invariance correspondence between different objects. The corresponding points, visualized as \textcolor{darkgreen}{green} dots, show a resemblance to the keypoint-based manipulation methods~\citep{gao2021kpam, manuelli2019kpam}. kPAM~\citep{manuelli2019kpam} and kPAM-SC~\citep{gao2021kpam} use object keypoints to compose objectives and constraints in the optimization-based planning for manipulation and demonstrate generalization over large shape variations in a pick-and-place setting. However, these methods require the manual design of keypoints for each object category. Our method IMOP does not require any specification of keypoints or any other form of labeling. The visualized connections are obtained by simply thresholding the output of the invariance matcher network $f_\mathcal{C}$. 


\subsection{Real-Robot Manipulation via One-shot Sim-to-Real Transfer}

\textbf{Setup.} We evaluate the one-shot sim-to-real performance of IMOP using simulation demonstrations for the base tasks, and trajectories recorded in the real-world as the one-shot demonstrations of novel tasks. We adopt five novel tasks: \textit{put toy in bowl}, \textit{stack blocks}, \textit{put item in shelf}. Contrary to existing work that requires over 10 demonstrations per task for re-training~\citep{goyal2023rvt}, the one-shot generalization capability of IMOP enables the sim-to-real transfer using only one demonstration and without re-training. We deploy the model on a Kuka LBR iiwa robot. We use RBG-D observations from a single RealSense D415 camera. We use  MoveIt~\citep{moveit} for planning paths that move the arm to the gripper poses predicted by IMOP.

% To simplify the study, we assume the first states of each episode of a given task are semantically equivalent. Therefore, the $i$ in line 6 of Algorithm~\ref{alg:eval} can be directly set to 0. We focus on the one-shot sim-to-real capacity of the invariance estimator $f_\mathcal{I}$ and matcher $f_\mathcal{C}$. 


\begin{table}[!htp]\centering
\caption{One-shot sim-to-real transfer performance of IMOP for solving real-world manipulation tasks.} \label{tab:real-robot-exp}
\begin{tabular}{lc}\toprule
Task & Success Rate \\\midrule
Put toy in bowl &80\% \\
Stack blocks &80\% \\
Put item in shelf &40\% \\
\bottomrule
\end{tabular}
\end{table}

\textbf{Result.} Table~\ref{tab:real-robot-exp} shows the success rate of IMOP on the five real-world tasks. The success rate of each task is the average of independent 10 runs with different object layouts. Figure~\ref{fig:real-robot-exp} visualizes the invariance correspondence between demonstration and test scenes. The sim-to-real gap is commonly acknowledged as a challenging problem in deploying control policies trained with simulation data~\citep{zhao2020sim}. In our study, we find that the invariance matcher $f_\mathcal{C}$ is robust to this domain shift. However, the output of the invariance estimator, $\widehat{\mathbf{P}}[p \in \mathcal{I}(s_i)]$, has much smaller values than those from simulation data. Thus, simply thresholding this probability with 0.5, as done in line 8 of Algorithm~\ref{alg:eval}, does not produce a valid invariant region. Instead, we circumvent this problem by using a much smaller threshold, $0.1$. 
The low success rate (40\%) on the `put item in shelf' task is likely due to the unstable invariant region estimation. This indicates that IMOP has the one-shot sim-to-real capacity, but still suffers from the sim-to-real gap for the invariant region estimation. This issue can potentially be addressed by fine-tuning with a small set of real-robot demonstrations, or simply using more cameras to improve the point cloud quality of complex objects, as RLBench has 4 cameras in the simulation setup but our real-robot setup only has a single camera.
% If still no valid regions can be found, as we have observed in the `put item in shelf' task, we cluster the points of current scene into segments using hdbscan, and predict the segment with the largest sum of probability $\widehat{\mathbf{P}}[p \in \mathcal{I}(s_i)]$ as the invariant region.






\subsection{Ablation Studies}
\label{sec:exp-analysis}





\begin{table}[!htp]\centering
\caption{Ablation studies on the components of IMOP.}\label{tab:ablation}
% \vspace{-1em}
\resizebox{\linewidth}{!}{
\begin{tabular}{ccc|cc}\toprule
Semantically &Regression by &Invariance &\multicolumn{2}{c}{Success Rate (\%)} \\
Equivalent State &Correspondence &Estimation &Base &Novel \\\midrule
\cmark &\cmark & &6.7 &- \\
&\cmark &\cmark & 65.7 & 38.8 \\
\cmark & &\cmark &58.2 &29.4 \\\midrule
\cmark &\cmark &\cmark &69.6 &41.3 \\
\bottomrule
\end{tabular}}
\end{table}

We study the component effects of IMOP in Table~\ref{tab:ablation}. The first row denotes the setting where the model does not estimate invariant regions but directly finds correspondences over the entire scene. The target end-effector pose is derived in Equation~\ref{eq:solve} by replacing $\mathcal{I}(s_i)$ and $\mathcal{I}(s_j)$ with $s_i$ and $s_j$. The model almost fails to predict actions on all tasks. This emphasizes the importance of estimating invariant regions. 
% --------- 
The second row of Table~\ref{tab:ablation} denotes the setting where we use the state pairs from $\mathcal{D}_{align}$ instead of $\mathcal{D}_{pair}$ to train invariance estimator $f_\mathcal{I}$ and matcher $f_\mathcal{C}$ as done in line 3 of Algorithm~\ref{alg:train}. This means the state pairs used in training are not necessarily semantically equivalent and therefore noisy. Note that we still use $\mathcal{D}_{pair}$ to train state matcher $f_\mathcal{S}$ in this setting. Contrary to the first setting, where success rates completely dropped, the success rate on both base and novel tasks decreases by only about 4\%, which still keeps IMOP's performance above the other baselines. This shows that having cleaner data improves performance but the training of IMOP is noise-tolerant to a certain extent. 

% --------- 
The third row of Table~\ref{tab:ablation} represents the setting where a conventional 3D pose regressor is used instead of predicting target poses by solving the least-squares problem in Equation~\ref{eq:solve}. For the conventional regressor, we use a similar architecture to Act3D~\citep{gervet2023act3d}. To measure the component effect more accurately, we keep the correspondence prediction branch and add the conventional 3D regression as a separate head. The success rate on both base and novel tasks decreases by about 10\% but the relative decrease on novel tasks is larger. This shows that predicting correspondences is a novel and accurate approach for 3D pose regression and has a stronger generalization ability. 


==> modules.backup/7.ending.tex <==
\section{Discussion and Conclusion}

We have shown that one-shot novel task generalization can be achieved by learning to estimate and match key invariant regions in the demonstration and test scene. This invariant region information is embedded in offline demonstrations, can be extracted via our proposed unsupervised procedure, and serves as supervision for network learning. The target end-effector pose can be transferred between semantically equivalent scenes by finding correspondences between invariant regions. Some open questions are, however, still worth discussing. The offline invariant region estimation procedure is designed for the simulated environment of RLBench. For real-world data, more sophisticated data preprocessing may be necessary, such as the use of open-set object detectors~\citep{zhang2023detect, zhong2022regionclip}. Despite the generality of our invariance-matching framework, the current definition of the invariant region is still closely linked to rigid body transformation. This suggests the potential for extending the formulation of invariant regions based on more general motion descriptors, such as warping or flows~\citep{li2022lepard}, to improve the manipulation accuracy on non-rigid objects.



With the emergence of neural architectures that are scalable to Internet-scale data~\citep{brown2020language}, 
the possibility of learning invariant regions from unlabeled human videos that are widely available has yet to be fully explored. Beyond only leveraging consecutive states to estimate invariant regions, it is possible to incorporate long-term information from multiple state transitions to further improve the manipulation performance.






==> modules/backup/method.jan22.tex <==
\section{An Invariance Perspective}
\label{sec:inv-p}

% direct

% remove the `challenging` 

% shorten the first paragraph.

% in input and output space of supervised learning task

Invariance is an inherent concept for machine learning.
In supervised learning, 
let $\mathcal{X}$ and $\mathcal{Y}$ denote the input and output space, and $y(x) \in \mathcal{Y}$ denote the category of $x \in \mathcal{X}$, $\mathcal{X}^{\mathcal{X}}$ denote the set of all functions from $\mathcal{X}$ to $\mathcal{X}$. 

% We view the existing work on one-shot learning through the concept of invariance, which in our perspective, constitutes an inherent structure for foundational one-shot learning work. Based on the concept of invariance, we formulate the one-shot manipulation problem into a tractable form and naturally motivate our algorithm as in Section~\ref{sec:one-shot-manipulation}. 


% change this to a definition
\begin{definition} Let $\mathcal{G} = \{g | y(x) = y(g(x)), \forall g \in \mathcal{X}^{\mathcal{X}} \}$ represents the set that includes all intra-class transformations on $\mathcal{X}$.
\label{asm:intra-trans}
\end{definition}

\begin{definition}
A function $f: \mathcal{X} \mapsto \mathbb{R}^n, n \in \mathbb{N}^+$ is invariant if $f(x) = f(g(x)), \forall x \in \mathcal{X}, g \in \mathcal{G}$.  
\label{def:inv}
\end{definition}

 
A perfect classifier $f(x)$ is an invariant function with $f(x_1) \neq f(x_2)$ such that $y(x_1) \neq y(x_2)$. $\mathcal{G}$ is implicitly represented through intra-class variations among samples over predefined categories $\mathcal{Y}^{b}$. One-shot learning enables the classification of novel categories $\mathcal{Y}^{n}$ by comparing input $x$ with a support sample $s$ such that $y(s) \in \mathcal{Y}^{n}$. Similar to supervised learning, we have Proposition~\ref{prop:osc}.

% put s in subscript

% define more clearly
% f(x) is not a function, is the value of the function

\begin{proposition}
If a function $f_s : \mathcal{X} \mapsto \{0, 1\}$ where $s \in \mathcal{X}, y(s) \in \mathcal{Y}^n$ is a perfect one-shot classifier, then  $f_s$ is an invariant function.  
\label{prop:osc}
\end{proposition}

However, this necessary invariant condition raises a significant challenge for one-shot learning. Since $s$ is the only sample available for novel category $\mathcal{Y}^n$, $\mathcal{G}$ can not be sufficiently represented for $x \in \mathcal{X}$ such that $y(x) \in \mathcal{Y}^n$ as in supervised learning. To this challenge, we introduce structures into a one-shot classifier $f_s$ by defining two functions: \emph{invariance encoder} $e : \mathcal{X} \mapsto \mathbb{R}^n$ and \emph{invariance matcher} $m: \mathbb{R}^n \times  \mathbb{R}^n \mapsto \mathcal{Y}$, where $e(x)$ is an invariant function.

\begin{proposition}
$f_s(x) := m(e(x), e(s))$ is an invariant function.  
\label{prop:inv}
\end{proposition}

% by only training on base categories where $\mathcal{G}$ is sufficiently represented

Instead of relying on the intra-class transformation $\mathcal{G}$ that is unavailable in the one-shot setting, the structure in Proposition~\ref{prop:inv} attempts to acquire the ability to capture and compare $\mathcal{G}$-invariant information.
We find this structure to inherently exist in many foundational one-shot learning works. 
Matching network~\citep{vinyals2016matching} captures invariance through extracting full-context embedding and comparing them through the matching network.
 Computing mean features as class representatives, a widely adopted strategy proposed by Prototypical network~\citep{snell2017prototypical}, accentuates invariant information.  
This structure brings forth the general ability to capture invariance as a key pathway to one-shot learning. In Section~\ref{sec:one-shot-manipulation}, we explain how the one-shot manipulation problem, despite challenging, is made approachable from this perspective.


%%%%%%%

\section{One-Shot Robotic Manipulation}
\label{sec:one-shot-manipulation}

\subsection{Problem Formulation}

We formalize the environment as a Markov Decision Process (MDP) represented by 5-tuple $\mathcal{M} = (\mathcal{S}, \mathcal{A}, P, R, \mu)$. $\mathcal{S}$ and $\mathcal{A}$ are the state and action space, $P: \mathcal{S}\times\mathcal{A} \mapsto \mathcal{S}$ is the state transition probability, $R: \mathcal{S} \mapsto \mathbb{R}$ denotes the reward function, and $\mu$ is the initial state distribution. During training, we assume the access to an offline dataset $\mathcal{D}$, and each trajectory $\tau_{base} = (s_0, a_0, r_0, ..., s_H, a_H, r_H), \tau_{base} \in \mathcal{D}$ is collected from a set of base tasks $\mathbf{T}^{base}$, where  $s_i \in \mathcal{S}, a_i \in \mathcal{A}$, $r_i$ is the per-timestamp reward, and $H$ is the episode length. The policy is evaluated on both $\mathbf{T}^{base}$ and a set of novel tasks $\mathbf{T}^{novel}$, which is disjoint to $\mathbf{T}^{base}$. During testing, we assume the access to a single successful trajectory $\tau_{novel}$ as a demonstration for each task in $\mathbf{T}^{novel}$. The objective is to build a one-shot policy $\pi(a | s, \tau), \tau \in \mathbf{T}^{base} \cup \mathbf{T}^{novel}$ that works in both base and novel tasks.



In robotics manipulation, $s \in \mathcal{S}$ is commonly represented as point clouds with each point $p_i \in s, i \in \{1, .., |s|\}$ is in homogenous coordinate as $p \in \mathbb{R}^4$, $|s|$ denotes the number of points, reward $R$ is sparse and only carries a binary success indicator in $r_H$, 
and $a \in \mathcal{A}$ represents a pose-level action, \emph{e.g.}, move the gripper to a given position.  Low-level robot movements are generated using off-the-shelf motion planners. RLBench requires an 8-dimensional action, including the 6-DoF end-effector pose (3-DoF for translation and 3-DoF for rotation), two binary indicators for gripper state (open or close), and whether to allow collision for the motion planner to handle tasks involving pushing.



\subsection{Algorithm}
\label{sec:algo}

\begin{figure*}
  \includegraphics[width=\textwidth]{assets/main-Page-1.drawio.png}
  \label{fig:method}
  \vspace{-2em}
  \caption{Illustration of our framework.}
\end{figure*}

Our algorithm is motivated by the question: How can the action $a$ be transferred from a state transition $(s, a, s') \in \tau$ to a query state $s^q$? This question necessitates a dichotomy understanding of actions. On the one hand, actions can be represented at the geometric level, using only translation and rotation of the end-effector.
Actions in this representation can be directly executed by robots.
If we denote $T_{s'}$ to be the homogenous transformation matrix of the end-effector pose in $s'$, then $a$ is equivalent to $T_{s'}$ and we write $a = T_{s'}$, \emph{i.e.}, the action on $s$ is the target end-effector pose $T_{s'}$. Note we focus on the end-effector pose in $a \in \mathcal{A}$, as the binary prediction part can be modeled with existing one-shot classification methods.

On the other hand, actions can be represented at a much higher semantic level. For example, holding a cup is a valid action regardless of the position or style of the cup. Actions in this representation cannot be directly executed by robots or even be exhaustively enumerated, but they carry clear semantic meaning and generalize across various scenes. Since $a$ is bound to its state $s$, we denote $A_s$ to be the semantic representation of $a$ on state $s$ and the action can only be transferred if $A_s = A_{s^q}$. In doing so, the above question is formulated into building a one-shot policy $\pi(T_{s^{q'}} | s^q, (s, s'))$, on which $\pi(a|s, \tau)$ can be composed by routing the query state to the closest state in the demonstration.
Driven by the invariance perspective in Section~\ref{sec:inv-p}, the following questions naturally arise: 

\begin{enumerate}
    % \item (\emph{state routing}) How to determine the matching between $s^q$ and $s^{sup}$?
    \item (\emph{invariance encoder}) How to discover the invariance within $s^q$ and $(s, s')$?
    \item (\emph{invariance matcher}) How to derive the $T_{s^{q'}}$ using $T_{s'}$ and the invariance discovered?
\end{enumerate}


\begin{definition}
The invariant region on state $s$ is $\mathcal{I}(s) = \{ p | p \in s;   \exists q \in x, \parallel T^{-1}_{s'} \cdot p  -  T^{-1}_{x'} \cdot q \parallel < \epsilon, \forall x \in \mathcal{S}, A_s = A_x, \}$, where $s'$ and $x'$ denote the next state of $s$ and $x$.
\label{def:invariance-ps}
\end{definition}


In light of the dichotomy understanding of actions, we propose to capture invariance as the \emph{invariant region} $\mathcal{I}(s)$ in Definition~\ref{def:invariance-ps}. Intuitively speaking, the low-level geometric action $T_{s'}$, \emph{i.e.}, the target end-effector pose, can be interpreted as an instantiation of a high-level semantic action $A_s$. The Definition~\ref{def:invariance-ps} assumes that a specific region $\mathcal{I}(s)$ can be found for the same semantic action $A_{s}$ across different scenes, whose coordinates under the low-level geometric action frame $T_{s'}$ are invariant. $\mathcal{I}(s)$ captures this invariant region in the form of a point set. 
We provide illustrative examples of $\mathcal{I}(s)$ in Figure~\ref{fig:method} and Figure~\todo{xx}.


\begin{definition}
The invariance correspondence between $s$ and $x$ is $\mathcal{C}(s, x) = \{(p, q) | q = \argmin_{q \in \mathcal{I}(x)} \parallel T^{-1}_{s'} \cdot p  -  T^{-1}_{x'} \cdot q \parallel, \forall p \in \mathcal{I}(s) \}$.
\label{def:invariance-corr}
\end{definition}


Unlike the common feature comparison techniques in one-shot learning, we discover our proposed \emph{invariant region} naturally leads to a matching procedure that derives $T_{s^{q'}}$, by finding \textit{invaraince corresondence} $\mathcal{C}(s, x)$ as in Definition~\ref{def:invariance-corr}. $\mathcal{C}(s, x)$ captures the point-level mapping with the minimal pairwise distance in the end-effector frame and can be computed given the $\mathcal{I}(s), \mathcal{I}(x)$ and $T_{s'}, T_{x'}$. Conversely, to transfer action from $(s, s')$ to $s^q$, if the correspondence is given, then $T_{s^{q'}}$ can be analytically solved in Equation~\ref{eq:solve} through least square:

\begin{equation}
\min\limits_{T_{s^{q'}}} \parallel T_{s^{q'}} \cdot T^{-1}_{s'} \cdot
 P_{\mathcal{I}(s)} \cdot C - P_{\mathcal{I}(s^q)} \parallel 
\label{eq:solve}
\end{equation}

where we use $P_{\mathcal{I}(s)} \in \mathbb{R}^{4\times |\mathcal{I}(s)|}$ to denote the points in $\mathcal{I}(s)$ and $C \in \mathbb{R}^{|\mathcal{I}(s)| \times |\mathcal{I}(s^q)|}$ to denote the assignment matrix equivalent to $\mathcal{C}(s, s^q)$ that $C_{ij} = \mathbb{I}[(p_i, q_j) \in \mathcal{C}(s, s^q)], \forall i \in \{1, .., |\mathcal{I}(s)|\}, j \in \{1, .., |\mathcal{I}(s^q)|\}$.



\begin{minipage}{\columnwidth}
\begin{algorithm}[H]
   \caption{IMOP Training}
   \label{alg:train}
\begin{algorithmic}[1]
   \STATE {\bfseries Input:} invariant region $\mathcal{I}$ and invariance correspondence $\mathcal{C}$, matched state pairs $\mathcal{D}_{pair}$, invariance encoder $e_{\theta}(s, s')$ and matcher $m_\theta(s, x, I)$
   
   \REPEAT
   \STATE Sample a state pair $(s^q, (s, s'))$ from $\mathcal{D}_{pair}$
   \STATE $\widehat{\mathbf{P}}[p \in \mathcal{I}(s)] \leftarrow e(s, s')$
   \STATE $I \leftarrow \mathbb{I}[p \in \mathcal{I}(s)]$.
   \STATE $\widehat{\mathbf{P}}[(p, q) \in \mathcal{C}(s, x)] \leftarrow m(s, x, I)$
   
   \STATE $\mathcal{L}_e \leftarrow \mathcal{L}_{focal}\left(\widehat{\mathbf{P}}[p \in \mathcal{I}(s)], \mathcal{I}(s)\right)$
   
   \STATE $\mathcal{L}_m \leftarrow \mathcal{L}_{focal}\left(\widehat{\mathbf{P}}[(p, q) \in \mathcal{C}(s, x)], \mathcal{C}(s, x)\right)$
   
   \STATE Update $\theta$ with backpropagation from $\mathcal{L}_e + \mathcal{L}_m$
   \UNTIL{converged}
\end{algorithmic}
\end{algorithm}
\end{minipage}
\begin{minipage}{\columnwidth}
\begin{algorithm}[H]
   \caption{IMOP Inference}
   \label{alg:inference}
\begin{algorithmic}[1]
   \STATE {\bfseries Input:} invariance encoder $e_{\theta}(s, s')$ and matcher $m_\theta(s, x, I)$, query state $s^q$, support state $(s, s')$
   % \STATE $(s, s') \leftarrow$ find  state closest to $s^q$ in $\tau$  
   \STATE $I \leftarrow \mathbb{I}[e(s, s') > 0.5]$
   \STATE $C \leftarrow m(s, s^q, I)$
   \STATE $\widehat{\mathcal{I}}(s) \leftarrow \{p_i | I_i = 1, i \in \{1, .., |s|\}\}$
   \STATE Solve $T_{s^{q'}} = \argmin_{T_{s^{q'}}} \parallel T_{s^{q'}} \cdot T_{s'}^{-1} \cdot P_{\widehat{\mathcal{I}}(s)} \cdot C - P_{s^q} \parallel$
   \STATE Return $T_{s^{q'}}$
\end{algorithmic}
\end{algorithm}
\end{minipage}

% $\mathcal{I}(a, s)$ can be obtained by thresholding the probability, \textit{e.g.}, $\mathbb{I}[e_\theta(s, a, s') > 0.5]$. 

To implement the above ideas, the enumeration of semantic action $A_s$ is required, which involves labor-intensive human annotation. Instead, we propose an unsupervised statistical approach to empirically estimate \textit{invariant region} $\mathcal{I}(s)$ in offline demonstrations, and determining the equality between $A_s$ and $A_x$ by checking whether a proper $\mathcal{C}(s, x)$ can be established. We detail our offline dataset construction in Section~\ref{sec:impl}. With the estimated $\mathcal{I}(s)$ and a dataset of matched state pairs $\mathcal{D}_{pair} = \{(s^q, (s, s')) | A_s = A_{s^q}), \exists \tau_1, \tau_2 \in \mathcal{D}, s \in \tau_1, s^q \in \tau_2 \}$, we obtain the policy  $\pi(T_{s^{q'}} | s^q, (s, s'))$ through a supervised learning setup.
% $\pi(T_{s^{q'}} | s^q, (s, s'))$

Specifically, we design the \emph{invariance encoder} as $e_\theta(s, s'): \mathcal{S} \times \mathcal{S} \mapsto [0, 1]^{|s|}$ to estimate the pointwise probability $\mathbf{P}[p_i \in \mathcal{I}(s)], i \in \{1, .., |s|\}$ from the start and end state of the action $A_s$. 
$\theta$ denotes network parameters.
%
We design the \emph{invariance matcher} as $m_\theta(s, x, I): \mathcal{S} \times \mathcal{S} \times \{0, 1\}^{|s|} \mapsto [0, 1]^{|\mathcal{I} \times |x|}$ to predict a soft corresondent matrix $C$ whose $C_{ij}$ denotes the pairwise probability $\mathbf{P}[(p_i, q_j) \in \mathcal{C}(s, x)], \forall i \in \{1, .., |\mathcal{I}(s)|\}, j \in \{1, .., |x|\}$. 
$m_\theta(s, x, I)$ uses $\mathcal{I}(s)$ to find and correspond to $\mathcal{I}(x)$ at the same time. We use $I$ to denote the binary mask that indicates whether $p_i \in \mathcal{I}(s), i \in \{1, .., |s|\}$.
In doing so, we present the invariance matching one-shot policy (IMOP).  We summarize the training and inference of IMOP in Algorithm~\ref{alg:train} and Algorithm~\ref{alg:inference}. 
We use focal loss between the probability estimation and $\mathcal{I}(s)$ and $\mathcal{C}(s, x)$. In practice, we match the support state $(s, s')$ for the first query state using a binary classification network trained with $\mathcal{D}_{pair}$. The following query states are matched with the rest of the demonstration $\tau$ accordingly. For the two binary indicators of gripper state and collision avoidance, we follow a nearest-neighbor classifier approach and use the corresponding values of $s$ as predictions for $s^q$.
Different to Equation~\ref{eq:solve}, the line 5 in Algorithm~\ref{alg:inference} use estimated invariant region $\widehat{\mathcal{I}}(s)$ and corresponds to the entire $s^q$ instead of $\mathcal{I}(s^q)$.




\subsection{Implementation Details}
\label{sec:impl}

\subsubsection{Offline Invariance Estimation}

We adopt a statistical approach to estimate \textit{invariant region} $\mathcal{I}(s)$. The intuition is that, since there are multiple trajectories in $\mathcal{D}$ for each base task if we transform the coordinate to the end-effector frame and estimate the point movements on similar states across different trajectories, the points with the least amount of movements belong to $\mathcal{I}(s)$. 



Specifically, we first build an initial set of matched state pairs $\mathcal{D}_{pair}^{0} = \{(s_i, x_i) |  s_i \in \tau_3, x_i \in \tau_2, \forall \tau_1, \tau_2 \in \mathbf{T}^{base}, \tau_1 \neq \tau_2, \textbf{T}(\tau_1) = \textbf{T}(\tau_2), i \in \{1, ..., |\tau_1|\}\}$ by interpolating all trajectories to the same length, \emph{i.e.}, $|\tau_1| = |\tau_2|, \forall \tau_1, \tau_2 \in \mathbf{T}^{base}$ and matching the states in the corresponding position for every two trajectories under each task. We denote $\textbf{T}(\tau)$ as the task of trajectory $\tau$.
Then, we estimate the expected movement of a point $p \in s$ by $\delta(p, s) = \mathbf{E}_{(s, x) \in \mathcal{D}_{pair}^0, q \in x} [\min \parallel T_{s'}^{-1} p - T_{x'}^{-1} q \parallel]$. Next, we cluster the points in state $s$ into segments $\{c_1, ..., c_n\}$ where each segment $c_i$ consists of a set of points. We estimate the \textit{invariant region} as the segment with the minimal expected movement $\mathcal{I}(s) = \argmin_{c_i} \mathbf{E}_{p \in s, p \in c_i} [\delta(p, s)]$. 


Using $\mathcal{I}(s)$, $\mathcal{C}(s, x)$ can be directly computed with the equation in Definition~\ref{def:invariance-corr}. We filter out the state pairs whose expected distances on corresponded points $\mathbf{E}_{(p, q) \in \mathcal{C}(s, x)} \parallel T^{-1}_{s'} \cdot p  -  T^{-1}_{x'} \cdot q \parallel$ are larger than a threshold, and the remaining state pairs compose $D_{pair}$.


\subsubsection{Network Architecture}



\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{assets/arch.drawio.png}
    \caption{caption}
    \label{fig:network}
\end{figure}


%  we use $\mathbf{E}$ to denote expectation, 
% todo: network architecture + a small graph

% the closest state in demonstration is found by selecting the one with maximal per-point correspondence probability.
% to speed up, we select the first frame and match following frames accordingly.



==> modules/backup/method.jan23.tex <==
\section{One-shot Imitation Learning with Invariance Matching}
\label{sec:method}

\subsection{Problem Formulation}

We denote $\mathbf{T}$ as the task space and formalize the environment for each task $t \in \mathbf{T}$ as a Markov Decision Process (MDP) represented by 5-tuple $\mathcal{M}_t = (\mathcal{S}, \mathcal{A}, P, R_t, \mu_t)$. $\mathcal{S}$ and $\mathcal{A}$ are the state and action spaces, $P:\mathcal{S}\times\mathcal{A}\mapsto\mathcal{S}$ is the state transition probability, $R_t: \mathcal{S}\mapsto\mathbb{R}$ denotes the reward function, and $\mu_t$ is the initial state distribution. During training, we assume the offline access to a dataset $\mathcal{D}_{base} = \{(s_i, a_i, s_{i+1})\}_{i=1}^{H_{base}}$, where $H_{base}$ denotes the number of transitions. $\mathcal{D}_{base}$ is collected from demonstrations on a set of base tasks $\mathbf{T}^{base}$. $\mathcal{D}_{base}$ does not include reward because $R_t$ is not available in the manipulation setting. During testing, we assume the offline access to a complete and successful trajectory $\tau_t = \{(s_i, a_i, s_{i+1})\}_{i=1}^{H_{\tau_t}}$ for each task $t$, where $H_{\tau_t}$ denotes the number of transitions. We refer to $\tau_t$ as the demonstration trajectory. Each task $t$ comes from $\mathbf{T}^{base} \cup \mathbf{T}^{novel}$, where $\mathbf{T}^{novel}$ represents a set of novel tasks that is disjoint to $\mathbf{T}^{base}$.  The goal is to build a one-shot policy $\pi(a | s, \tau_t)$, a multi-task policy that works in both base and novel tasks given a demonstration trajectory, and does not require any finetuning.

In a robotic manipulation task, $s \in \mathcal{S}$ is commonly represented as point cloud of the whole scene including the robot, with each point $p_i \in s, i \in \{1, ..., |s|\}$ in homogeneous coordinate, $|s|$ denotes the number of points. $a \in \mathcal{A}$ represents a pose-level action, \textit{e.g.}, move the end-effector to a given position and close the gripper. Low-level robot movements are generated using off-the-shelf motion planners. For example, RLBench~\citep{james2020rlbench} an 8-dimensional action, including the 6-DoF end-effector pose (3-DoF for translation and 3-DoF for rotation), two binary indicators for gripper state (open or close, whether to allow collision). We write $a = (T_a, \lambda_a)$ to decompose action into two components, where $T_a \in \mathbb{R}^{4\times4}$ denotes the target end-effector pose in homogenous matrix form, and $\lambda_a$ denotes the binary values of gripper state. 

\subsection{Central Idea}

We first consider a sub-problem: given an observed transition $(s_i, a_i, s_{i+1})$ and a new state $s_j$, assuming $s_i \equiv s_j$, how to derive the $T_{a_j}$? We write $s_i \equiv s_j$ to denote $s_i$ is semantically equivalent to $s_j$. The semantical equivalence is a loose notion here and we will address it later. To solve this problem, we define the \textbf{invariant region} in Definition~\ref{def:inv}.

\begin{definition}
    The invariant region in $s_i$ is $\mathcal{I}(s_i) = \{ p | p \in s_i, \forall s_j \in \mathcal{S}, s_i \equiv s_j, 
\exists q \in s_j: \parallel T^{-1}_{a_i} p - T^{-1}_{a_j} q \parallel < \epsilon \}$.
\label{def:inv}
\end{definition}

$\mathcal{I}(s_i)$ is a set of points, whose coordinates remain invariant across all states semantical equivalent to $s_i$, when viewed in the target end-effector frame $T_{a_i}$. Take the example of picking up a cup, the action is usually to grasp the cup handle, regardless of the location, orientation, or style of the cup. The invariant region in this example is likely to be the cup handle area. Based on the invariant region, $T_{a_j}$ can be obtained through finding correspondence between $\mathcal{I}(s_i)$ and $\mathcal{I}(s_j)$. We define the \textbf{invariance correspondence} in Definition~\ref{def:corr}.

\begin{definition}
The invariance correspondence between $s_i$ and $s_j$ is $\mathcal{C}(s_i, s_j) = \{(p, q) | q = \argmin_{q\in \mathcal{I}(s_j)} \parallel T^{-1}_{a_i} p - T^{-1}_{a_j} q \parallel, p \in \mathcal{I}(s_i)\}$.
\label{def:corr}
\end{definition}

$\mathcal{C}(s_i, s_j)$ is a set of point-level mappings that produce the minimal pairwise distance between the points in $\mathcal{I}(s_i)$ and $\mathcal{I}(s_j)$, when transformed to the end-effector frame $T_{a_i}$ and $T_{a_j}$, respectively. This means that if $\mathcal{C}(s_i, s_j)$ is given, then $T_{a_j}$ can be analytically solved by the optimization problem in Equation~\ref{eq:solve} with a least square algorithm~\citep{huang1986least}.

\vspace{-1em}

\begin{equation}
\min_{T_{a_j}} \parallel T_{a_j} T^{-1}_{a_i}  P_{\mathcal{I}(s_i)}  C - P_{\mathcal{I}(s_j)} \parallel
\label{eq:solve}
\end{equation}

where $P_{\mathcal{I}(s)} \in \mathbb{R}^{4 \times |\mathcal{I}(s)|}$ denotes the points in $\mathcal{I}(s)$, $C \in \{0, 1\}^{|\mathcal{I}(s_i)| \times |\mathcal{I}(s_j)|}$ denote the assignment matrix equivalent to $\mathcal{C}(s_i, s_j)$ where $C_{mn} = 1$ if $(p_m, q_n) \in \mathcal{C}(s_i, s_j)$ and vice versa. Whereas Equation~\ref{eq:solve} provides a solution to derive $T_{a_j}$, how to determine $\mathcal{I}(s_i)$ and semantical equivalent states remain unsolved. We address them in Section~\ref{sec:offline-inv-e}.


\subsection{Offline Invariance Estimation}
\label{sec:offline-inv-e}

We first consider the estimation of $\mathcal{I}(s_i)$ for the observed states in the offline dataset $\mathcal{D}_{base}$. One way is to manually build an action vocabulary and assign the labels to all states through annotation~\citep{gu2018ava}. $s_i$ is semantically equivalent to $s_j$ if they share the same action label. Then, $\mathcal{I}(s_i)$ can be solved through optimization with constraints $\parallel T^{-1}_{a_i} p - T^{-1}_{a_j} q \parallel < \epsilon, \forall s_i \equiv s_j$. However, manual annotation is label-intensive. Instead, we propose an unsupervised empirical approach to first get a noisy estimation of $\mathcal{I}(s)$ and $\mathcal{C}(s_i, s_j)$. Next, we solve $T_{a_j}$ using Equation~\ref{eq:solve} with the noisy estimation of $\mathcal{C}(s_i, s_j)$. 
An inferior estimation of $\mathcal{C}(s_i, s_j)$ leads to poor estimation of $T_{a_j}$. 
Since the groundtruth of $T_{a_j}$ is available in $\mathcal{D}_{base}$, we measure the estimation quality of $\mathcal{C}(s_i, s_j)$ by comparing the groundtruth and estimation of $T_{a_j}$. Finally, we remove the inferior estimations. We detail the procedure in the following.

To estimate $\mathcal{I}(s)$, we observe that there are 
multiple trajectories in $\mathcal{D}_{base}$ for each task.  We transform the coordinate of each state $s$ to the target end-effector frame $T_a$ and estimate the point movements on similar states across different trajectories. The points with the least amount of movements compose $\mathcal{I}(s)$. Specifically, let denote $\tau_k = \{(s_{k,i}, a_{k,i}, s_{k,i+1})\}_{i=1}^{H_{\tau_k}}, k \in [K]$ denote a trajectory for task $t$ in $\mathcal{D}_{base}$, where $K$ and $H_{\tau_k}$ denote the number and length of trajectories. Here we skip the task notation $t$ for clarity. Next, we build a set of state pairs $\mathcal{D}^0_{pair}$ in Equation~\ref{eq:pair0}.

\vspace{-1em}

\begin{nalign}
\mathcal{D}^0_{pair} = \{(s_{k_1,i_1}, s_{k_2, i_2}) | i_1 = \round{{i \cdot H_{\tau_{k_1}}}/{H_{max}}}, \\ 
i_2 =  \round{{i \cdot H_{\tau_{k_2}}}/{H_{max}}}, 
\\ i \in [H_{max}], H_{max} = \max(H_{\tau_{k_1}}, H_{\tau_{k_2}}), \\
\forall k_1, k_2 \in [K], k_1 \neq k_2 \}
\label{eq:pair0}
\end{nalign}

$\mathcal{D}^0_{pair}$ pairs state $s_{k_1, i_1}$ in $\tau_{k_1}$ to another state $s_{k_2, i_2}$ in $\tau_{k_2}$, where $i_1$ and $i_2$ are aligned accordingly. Then, we estimate the expected movement of a point $p \in s$ by $\Delta_{s}(p)$ in Equation~\ref{eq:delta}.

\begin{equation}
\Delta_{s_1}(p) = \mathbf{E}_{(s_1, s_2) \in \mathcal{D}^0_{pair}} \left[\min_{q \in s_2} \parallel T^{-1}_{a_1} p - T^{-1}_{a_2} q \parallel \right]
\label{eq:delta}
\end{equation}


Then, we cluster the points in state $s$ into segments $\{c_{s,n}\}_{n=1}^N$, where $N$ denotes the number of segments and each segment $c_{s,n} \subseteq s$ is a set of points.
We estimate the $\mathcal{I}(s)$ as the segment with the minimal expected movement as in Equation~\ref{eq:segment}.

\begin{equation}
\widehat{\mathcal{I}}(s) = \argmin_{c_{s, n}} \mathbf{E}_{p \in c_{s, n}} [\Delta_{s}(p)]
\label{eq:segment}
\end{equation}

where $\widehat{\mathcal{I}}(s)$ denotes the offline estimation of $\mathcal{I}(s)$. Next, we estimate the $\mathcal{C}(s_1, s_2)$ and $T_{a_2}$ through point-set registration as in Equation~\ref{eq:C-reg}.

\begin{equation}
\begin{gathered}
\left[\widehat{\mathcal{C}}(s_1, s_2), \widehat{T}_{s_1 \rightarrow s_2}\right] = \text{ICP}\left(\widehat{\mathcal{I}}(s_1), \widehat{\mathcal{I}}(s_2)\right) \\
\widehat{T}_{s_1 \rightarrow s_2, a_2} = \widehat{T}_{s_1 \rightarrow s_2} \cdot T_{a_1}
\end{gathered}
\label{eq:C-reg}
\end{equation}

where $\widehat{\mathcal{C}}(s_1, s_2)$ denotes the offline estimation of $\mathcal{C}(s_1, s_2)$, $\widehat{T}_{s_1 \rightarrow s_2}$ denotes the transformation that aligns $\widehat{\mathcal{I}}(s_1)$ to $\widehat{\mathcal{I}}(s_2)$. ICP denotes the iterative closest point algorithm~\citep{besl1992method}. $\widehat{T}_{s_1 \rightarrow s_2, a_2}$ denotes the target end-effector pose estimated from $s_1$ and $s_2$. Then, we measure the quality of the estimation by $Err(s_1, s_2)$ in Equation~\ref{eq:err}.

\begin{equation}
Err(s_1, s_2) = \parallel \widehat{T}_{s_1 \rightarrow s_2, a_2} - T_{a_2} \parallel 
\label{eq:err}
\end{equation}

Finally, we remove the pairs from $D^0_{pair}$ whose $Err(s_1, s_2)$ is larger than a threshold $\gamma$ as in Equation~\ref{eq:pair1}.

\begin{equation}
D_{pair} = \{ (s_1, s_2) | Err(s_1, s_2) \leq \gamma, (s_1, s_2) \in \mathcal{D}^0_{pair}\}
\label{eq:pair1}
\end{equation}

We consider $s_i \equiv s_j$ if $(s_i, s_j) \in D_{pair}$. Therefore, $\mathcal{I}(s)$, $\mathcal{C}(s_1, s_2)$, and semantical equivalent states are estimated. We detail how to train a one-shot policy based on $\widehat{\mathcal{I}}(s)$, $\widehat{\mathcal{C}}(s_1, s_2)$, and $\mathcal{D}_{pair}$ in Section~\ref{sec:algo}.

\subsection{Algorithm}
\label{sec:algo}

==> modules/backup/method.jan24.tex <==
\section{One-shot Imitation Learning with Invariance Matching}
\label{sec:method}

\subsection{Problem Formulation}

We denote $\mathbf{T}$ as the task space and formalize the environment for each task $t \in \mathbf{T}$ as a Markov Decision Process (MDP) represented by 5-tuple $\mathcal{M}_t = (\mathcal{S}, \mathcal{A}, \mathbf{P}, R_t, \mu_t)$. $\mathcal{S}$ and $\mathcal{A}$ are the state and action spaces, $\mathbf{P}:\mathcal{S}\times\mathcal{A}\mapsto\mathcal{S}$ is the state transition probability, $R_t: \mathcal{S}\mapsto\mathbb{R}$ denotes the reward function, and $\mu_t$ is the initial state distribution. During training, we assume the offline access to a dataset $\mathcal{D}_{base} = \{(s_i, a_i, s_{i+1})\}_{i=1}^{H_{base}}$, where $H_{base}$ denotes the number of transitions. $\mathcal{D}_{base}$ is collected from successful demonstrations on a set of base tasks $\mathbf{T}^{base}$. $\mathcal{D}_{base}$ does not include reward because $R_t$ is a binary success indicator function in the manipulation setting and only returns 1 at the last transition of a successful episode and 0 otherwise. During testing, we assume the offline access to a complete and successful trajectory $\tau_t = \{(s_i, a_i, s_{i+1})\}_{i=1}^{H_{\tau_t}}$ for each task $t$, where $H_{\tau_t}$ denotes the number of transitions. We refer to $\tau_t$ as the demonstration trajectory. Each task $t$ comes from $\mathbf{T}^{base} \cup \mathbf{T}^{novel}$, where $\mathbf{T}^{novel}$ represents a set of novel tasks that is disjoint to $\mathbf{T}^{base}$.  The goal is to build a one-shot policy $\pi(a | s, \tau_t)$, a multi-task policy that works in both base and novel tasks given a demonstration trajectory, and does not require any finetuning.

In a robotic manipulation task, $s \in \mathcal{S}$ is commonly represented as point cloud of the whole scene including the robot, with each point $p_i \in s, i \in \{1, ..., |s|\}$ in homogeneous coordinate, $|s|$ denotes the number of points. $a \in \mathcal{A}$ represents a pose-level action, \textit{e.g.}, move the end-effector to a given position and close the gripper. Low-level robot movements are generated using off-the-shelf motion planners. For example, RLBench~\citep{james2020rlbench} an 8-dimensional action, including the 6-DoF end-effector pose (3-DoF for translation and 3-DoF for rotation), two binary indicators for gripper state (open or close, whether to allow collision). We write $a = (T_a, \lambda_a)$ to decompose action into two components, where $T_a \in \mathbb{R}^{4\times4}$ denotes the target end-effector pose in homogenous matrix form, and $\lambda_a$ denotes the binary values of gripper state. 

\subsection{Central Idea}

We first consider a sub-problem: given an observed transition $(s_i, a_i, s_{i+1})$ and a new state $s_j$, assuming $s_i \equiv s_j$, how to derive the $T_{a_j}$? We write $s_i \equiv s_j$ to denote $s_i$ is semantically equivalent to $s_j$. The semantical equivalence is a loose notion here and we will address it later. To solve this problem, we define the \textbf{invariant region} in Definition~\ref{def:inv}.

\begin{definition}
    The invariant region in $s_i$ is $\mathcal{I}(s_i) = \{ p | p \in s_i, \forall s_j \in \mathcal{S}, s_i \equiv s_j, 
\exists q \in s_j: \parallel T^{-1}_{a_i} p - T^{-1}_{a_j} q \parallel < \epsilon \}$.
\label{def:inv}
\end{definition}

$\mathcal{I}(s_i)$ is a set of points, whose coordinates remain invariant across all states semantical equivalent to $s_i$, when viewed in the target end-effector frame $T_{a_i}$. Take the example of picking up a cup, the action is usually to grasp the cup handle, regardless of the location, orientation, or style of the cup. The invariant region in this example is likely to be the cup handle area. Based on the invariant region, $T_{a_j}$ can be obtained through finding correspondence between $\mathcal{I}(s_i)$ and $\mathcal{I}(s_j)$. We define the \textbf{invariance correspondence} in Definition~\ref{def:corr}.

\begin{definition}
The invariance correspondence between $s_i$ and $s_j$ is $\mathcal{C}(s_i, s_j) = \{(p, q) | q = \argmin_{q\in \mathcal{I}(s_j)} \parallel T^{-1}_{a_i} p - T^{-1}_{a_j} q \parallel, p \in \mathcal{I}(s_i)\}$.
\label{def:corr}
\end{definition}

$\mathcal{C}(s_i, s_j)$ is a set of point-level mappings that produce the minimal pairwise distance between the points in $\mathcal{I}(s_i)$ and $\mathcal{I}(s_j)$, when transformed to the end-effector frame $T_{a_i}$ and $T_{a_j}$, respectively. This means that if $\mathcal{C}(s_i, s_j)$ is given, then $T_{a_j}$ can be analytically solved by the optimization problem in Equation~\ref{eq:solve} with a least square algorithm~\citep{huang1986least}.

\vspace{-1em}

\begin{equation}
\min_{T_{a_j}} \parallel T_{a_j} T^{-1}_{a_i}  P_{\mathcal{I}(s_i)}  C - P_{\mathcal{I}(s_j)} \parallel
\label{eq:solve}
\end{equation}

where $P_{\mathcal{I}(s)} \in \mathbb{R}^{4 \times |\mathcal{I}(s)|}$ denotes the points in $\mathcal{I}(s)$, $C \in \{0, 1\}^{|\mathcal{I}(s_i)| \times |\mathcal{I}(s_j)|}$ denote the assignment matrix equivalent to $\mathcal{C}(s_i, s_j)$ where $C_{mn} = 1$ if $(p_m, q_n) \in \mathcal{C}(s_i, s_j)$ and vice versa. Whereas Equation~\ref{eq:solve} provides a solution to derive $T_{a_j}$, how to determine $\mathcal{I}(s_i)$ and semantical equivalent states remain unsolved. We address them in Section~\ref{sec:offline-inv-e}.


\subsection{Offline Invariance Region Estimation}
\label{sec:offline-inv-e}

We first consider the estimation of $\mathcal{I}(s_i)$ for the observed states in the offline dataset $\mathcal{D}_{base}$. One way is to manually build an action vocabulary and assign the labels to all states through annotation~\citep{gu2018ava}. $s_i$ is semantically equivalent to $s_j$ if they share the same action label. Then, $\mathcal{I}(s_i)$ can be solved through optimization with constraints $\parallel T^{-1}_{a_i} p - T^{-1}_{a_j} q \parallel < \epsilon, \forall s_i \equiv s_j$. However, manual annotation is labor-intensive. Instead, we propose an unsupervised empirical approach to directly estimate  $\mathcal{I}(s_i)$. Since the groundtruth value of $T_{a_j}$ is available in $\mathcal{D}_{base}$, we determine $s_i \equiv s_j$ based on the estimation error of $T_{a_j}$.



To estimate $\mathcal{I}(s_i)$, we first obtain a set of state pairs $\mathcal{D}_{match}$ through trajectory matching, which matches states from different trajectories of the same task in $\mathcal{D}_{base}$ based on trajectory length. We detail this procedure in Section~\ref{sec:impl-detail}. We measure the expected displacement of a point $p \in s_i$ by $\Delta_{s_i}(p)$ in the target end-effector frame by Equation~\ref{eq:delta}.

\vspace{-1.5em}
\begin{equation}
\Delta_{s_i}(p) = \mathbf{E}_{(s_i, s_j) \in \mathcal{D}_{match}} \left[\min_{q \in s_j} \parallel T^{-1}_{a_i} p - T^{-1}_{a_j} q \parallel \right]
\label{eq:delta}
\end{equation}

Then, we cluster the points in state $s_i$ into segments $\{c_{s_i,n}\}_{n=1}^N$, where $N$ denotes the number of segments and each segment $c_{s_i,n} \subseteq s_i$ is a set of points.
We define $\mathcal{I}(s_i)$ as the segment with the minimal expected displacement as in Equation~\ref{eq:segment}.

\vspace{-1em}

\begin{equation}
\mathcal{I}(s_i) = \argmin_{c_{s_i, n}} \mathbf{E}_{p \in c_{s_i, n}} [\Delta_{s_i}(p)]
\label{eq:segment}
\end{equation}


To determine $s_i \equiv s_j$, we align $\mathcal{I}(s_i)$ to $\mathcal{I}(s_j)$ through point-set registration, and compute the alignment error of the target end-effector pose as $err(s_i, s_j)$ in Equation~\ref{eq:C-reg}. 

\begin{equation}
\begin{gathered}
T_{\mathcal{I}(s_i) \rightarrow \mathcal{I}(s_j)} = \text{Align}\left(\mathcal{I}(s_i), \mathcal{I}(s_i)\right) \\
err(s_i, s_j) = \parallel T_{\mathcal{I}(s_i) \rightarrow \mathcal{I}(s_j)} T_{a_i}  - T_{a_j} \parallel
\end{gathered}
\label{eq:C-reg}
\end{equation}


where $T_{\mathcal{I}(s_i) \rightarrow \mathcal{I}(s_j)} \in \mathbb{R}^{4\times 4}$ denotes the alignment transformation, and the iterative closest point method~\citep{besl1992method} is used for alignment. We define $s_i \equiv s_j$ if $err(s_i, s_j) < \gamma$, where $\gamma$ is a hyper-parameter. In Equation~\ref{eq:dpair}, we define $D_{pair}$ to be the semantical equivalent state pairs in $D_{match}$.

\begin{equation}
D_{pair}=\{(s_i, s_j) | (s_i, s_j) \in \mathcal{D}_{match}, err(s_i, s_j) < \gamma \}
\label{eq:dpair}
\end{equation}

Whereas $\mathcal{I}(s_i)$ and semantical equivalent states are estimated in the offline dataset $\mathcal{D}_{base}$, how to determine $\mathcal{I}(s_i)$ in an observed transition $(s_i, a_i, s_{i+1})$ and new state $s_j$ during testing remains unsolved. We address them in Section~\ref{sec:algo}.  



\subsection{Algorithm}
\label{sec:algo}

We design neural networks that estimate invariant region $\mathcal{I}(s_i)$ from an observed transition $(s_i, a_i, s_{i+1})$, and predict $\mathcal{I}(s_j)$ of a new state $s_j$ through matching between $\mathcal{I}(s_i)$ and $s_j$. In doing so, we present the \textbf{I}nvariance \textbf{M}atching \textbf{O}ne-shot \textbf{P}olicy learning (IMOP).  We summarize the training and evaluation of IMOP in Algorithm~\ref{alg:train} and Algorithm~\ref{alg:eval}. We detail the procedure in the following. 

To estimate $\mathcal{I}(s_i)$, we design the invariance estimator function $f_{\mathcal{I}}: \mathcal{S}\times \mathcal{S}\times \Theta \mapsto [0, 1]^{|s_i|}$, where $\Theta$ denotes the network parameter space, and $|s_i|$ denotes the number of points in $s_i$. $f_{\mathcal{I}}$ takes $s_i, s_{i+1}$ as input and predict a pointwise probability $\widehat{\mathbf{P}}[p \in \mathcal{I}(s_i)]$ as in line 6 of Algorithm~\ref{alg:train}. The invariant region is obtained by thresholding this probability to a pointwise binary mask as in line 8 of Algorithm~\ref{alg:eval}. $f_{\mathcal{I}}$ is trained by focal loss~\citep{lin2017focal} with $\mathcal{I}(s_i)$ in the offline data as labels, as in line 13 of Algorithm~\ref{alg:train}.


To estimate $\mathcal{I}(s_j)$ and derive $T_{a_j}$, we design the invariance matcher function $f_\mathcal{C}: \mathcal{S} \times \mathcal{S} \times \{0, 1\}^{|s_i|} \times \Theta \mapsto [0, 1]^{|\mathcal{I}(s_i)| \times |s_j|}$, where $|\mathcal{I}(s_i)|, |s_i|$ and $|s_j|$ denote the number of points in $\mathcal{I}(s_i)$, $s_i$, and $s_j$, respectively.
$f_\mathcal{C}$ takes $s_i$, $s_j$ and $I_{s_i}$ as input and predicts a pairwise probability $\widehat{\mathbf{P}}[(p, q) \in \mathcal{C}(s_i, s_j)]$ as in line 8 of Algorithm~\ref{alg:train}, where $I_{s_i}$ denotes the binary mask representation of $\mathcal{I}(s_i)$. $f_{\mathcal{C}}$ is trained by focal loss with $\mathcal{C}(s_i, s_j)$ as labels, and $\mathcal{C}(s_i, s_j)$ is computed from $\mathcal{I}(s_i)$ and $\mathcal{I}(s_j)$ in the offline data, as in line 9 and 14 of Algorithm~\ref{alg:train}.
The output of $f_\mathcal{C}$ is a soft assignment matrix $C \in [0, 1]^{|\mathcal{I}(s_i)| \times |s_j|}$. The target end-effector pose $T_{a_j}$ of state $s_j$ can be solved by replacing $\mathcal{I}(s_j)$  with $s_j$ in Equation~\ref{eq:C-reg}, as in line 9 and 10 of Algorithm~\ref{alg:eval}. 


To determine whether $s_i \equiv s_j$ and derive the target gripper state $\lambda_{a_j}$, we design the state matcher function $f_\mathcal{S}:  \mathcal{S} \times \mathcal{S} \times \Theta \mapsto [0, 1]$. $f_\mathcal{S}$ takes $s_i$ and $s_j$ as input and predict the probability $\widehat{\mathbf{P}}[s_i \equiv s_j]$ as in line 10 of Algorithm~\ref{alg:train}. $f_{\mathcal{S}}$ is trained by focal loss with state pairs in $\mathcal{D}_{pair}$ as positive samples and random state pairs as negative ones, as in line 12 of Algorithm~\ref{alg:train}. In evaluation, $(s_i, a_i, s_{i+1}) \in \tau_t$ is chosen by the largest $\widehat{\mathbf{P}}[s_i \equiv s_j]$ for the first new state $s_j$, as in lines 3-6 of Algorithm~\ref{alg:eval}. $s_{i+1}$ is directly selected as the semantical equivalent state for the second new state and so on, as shown in lines 12-13 of Algorithm~\ref{alg:eval}. The target gripper state $\lambda_{a_i}$ of $s_i$ is used as the prediction for $\lambda_{a_j}$ in the new state $s_j$, as in line 11 of Algorithm~\ref{alg:eval}. An evaluation episode finishes when the task is completed with a reward of 1, or the demonstration trajectory $\tau_t$ has been consumed, as in line 14 of Algorithm~\ref{alg:eval}.



% \begin{minipage}{\columnwidth}
\begin{algorithm}
   \caption{IMOP Training}
   \label{alg:train}
\begin{algorithmic}[1]
   \STATE {\bfseries Input:} offline dataset $\mathcal{D}_{base}$,  invariant region $\mathcal{I}$, semantical equivalent state pairs $\mathcal{D}_{pair}$, state matcher $f_{\mathcal{S}}(s_i, s_j; \theta)$, 
   invariance estimator $f_{\mathcal{I}}(s_i, s_{i+1}; \theta)$, invariance matcher $f_\mathcal{C}(s_i, s_j, I_{s_i}; \theta)$, parameters $\theta$, 
   
   \REPEAT
   \STATE Sample a state pair $(s_i, s_j)$ from $\mathcal{D}_{pair}$

    \STATE Retrieve $(s_i, a_i, s_{i+1})$ and $(s_j, a_j, s_{j+1})$ from $\mathcal{D}_{base}$
    \STATE Randomly sample a state $s_k$ from $\mathcal{D}_{base}$

   \STATE $\widehat{\mathbf{P}}[p \in \mathcal{I}(s_i)] \leftarrow f_\mathcal{I}(s_i, s_{i+1}; \theta)$
   \STATE $I_{s_i} \leftarrow \mathbb{I}[p \in \mathcal{I}(s_i)]$.
   
   \STATE $\widehat{\mathbf{P}}[(p, q) \in \mathcal{C}(s_i, s_j)] \leftarrow f_\mathcal{C}(s_i, s_j, I_{s_i}; \theta)$

   \STATE Compute $\mathcal{C}(s_i, s_j)$ with Definition~\ref{def:corr} with $I_{s_i}, I_{s_j}$

   \STATE $\widehat{\mathbf{P}}[s_i \equiv s_j] \leftarrow f_\mathcal{S}(s_i, s_j;\theta)$
   \STATE $\widehat{\mathbf{P}}[s_i \equiv s_k] \leftarrow f_\mathcal{S}(s_i, s_k;\theta)$

   \STATE \scalebox{1}{$\mathcal{L}_{\mathcal{S}} \leftarrow \mathcal{L}_{\text{focal}}\big(\widehat{\mathbf{P}}[s_i \equiv s_k] , 0\big) + \mathcal{L}_{\text{focal}}\big(\widehat{\mathbf{P}}[s_i \equiv s_j], 1\big)$}
    
   
   \STATE $\mathcal{L}_\mathcal{I} \leftarrow \mathcal{L}_{\text{focal}}\big(\widehat{\mathbf{P}}[p \in \mathcal{I}(s_i)], \mathcal{I}(s_i)\big)$
   
   \STATE $\mathcal{L}_\mathcal{C} \leftarrow \mathcal{L}_{\text{focal}}\big(\widehat{\mathbf{P}}[(p, q) \in \mathcal{C}(s_i, s_j)], \mathcal{C}(s_i, s_j)\big)$
   
   \STATE Update $\theta$ with backpropagation from $\mathcal{L}_\mathcal{S} + \mathcal{L}_\mathcal{I} + \mathcal{L}_\mathcal{C}$
   \UNTIL{converged}
\end{algorithmic}
\end{algorithm}
% \end{minipage}
% \begin{minipage}{\columnwidth}
\begin{algorithm}
   \caption{IMOP Evaluation}
   \label{alg:eval}
\begin{algorithmic}[1]
   \STATE {\bfseries Input:} invariance estimator $f_{\mathcal{I}}(s_i, s_{i+1}; \theta)$, invariance matcher $f_\mathcal{C}(s_i, s_j, I_{s_i}; \theta)$, state matcher $f_{\mathcal{S}}(s_i, s_j; \theta)$, network parameters $\theta$, demonstration trajectory $\tau_t$, environment $\mathcal{M}_t$
   \STATE Sample initial state $s_j$ from $\mu_t$
   \FORALL{$(s_k, a_k, s_{k+1}) \in \tau_t$}
   \STATE $\widehat{\mathbf{P}}[s_k \equiv s_j] \leftarrow f_\mathcal{S}(s_k, s_j;\theta)$
   \ENDFOR
   \STATE $i \leftarrow \argmax_{k} \widehat{\mathbf{P}}[s_k \equiv s_j]$

   \REPEAT 
   \STATE $I_{s_i} \leftarrow \mathbb{I}[f_\mathcal{I}(s_i, s_{i+1}; \theta) > 0.5]$
   \STATE $C \leftarrow f_\mathcal{C}(s_i, s_j, I_{s_i})$
   \STATE Solve $T_{a_j} = \argmin_{T_{a_j}} \parallel T_{a_j} T_{a_i}^{-1} P_{I_{s_i}} C - P_{s_j} \parallel$
   \STATE $a_j \leftarrow (T_{a_j}, \lambda_{a_i})$
   \STATE Sample the next state $s_j$ from $\mathbf{P}(s | s_j, a_j)$
   \STATE $i \leftarrow i + 1$
   \UNTIL{$R_t(s_j) = 1$ \OR $i > |\tau_t|$}
\end{algorithmic}
\end{algorithm}
% \end{minipage}




\subsection{Implementation Details}
\label{sec:impl-detail}



We build $f_\mathcal{I}$, $f_\mathcal{S}$, and $f_\mathcal{C}$ using graph neural networks. Figure~\ref{fig:network} illustrates the network architectures. First, we extract point-level features using a point transformer network~\citep{zhao2021point} over the knn graphs on the point clouds of $s_i, s_{i+1}$ and $s_j$. 
Features of two granularities are represented as coarse points and fine points in Figure~\ref{fig:network}. 
Next, we apply transformers on knn graphs built between different point clouds. Take $f_{\mathcal{I}}$ for example, knn graphs between $s_i$ and $s_{i+1}$ are constructed to encourage the network to capture movement information. 
Notably, for $f_\mathcal{I}$ and $f_\mathcal{S}$, the knn graphs are built on coarse points to encourage interactions over larger spaces. Finally, the output of $f_\mathcal{I}$ and $f_\mathcal{S}$ are derived by applying a linear layer upon the point features. For $f_\mathcal{C}$, a cross attention layer is used between the point features of $\mathcal{I}(s_i)$ and $s_j$ to produce the probability matrix. 

Point transformer applies attention between the adjacent nodes of a graph and is more efficient than a traditional transformer because the degree of a graph is usually much smaller than the total number of nodes. The original point transformer only supports self-attention on graphs built from a single point cloud~\citep{zhao2021point}. We extend it to support cross-attention on knn graphs built from different point clouds. Our point transformer network is based on the PTv2~\citep{wu2022point} implemented in Pointcept~\citep{pointcept2023}, and PyTorch3D~\citep{ravi2020pytorch3d}. We use the soft Procrustes operator from Lepard~\citep{li2022lepard} to solve the least square problem in line 10 of Algorithm~\ref{alg:eval}. 


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{assets/arch.drawio.png}
    \caption{Network architectures of $f_\mathcal{I}$, $f_\mathcal{S}$, and $f_\mathcal{C}$.}
    \label{fig:network}
\end{figure}


% Trajectory Matching

% Appendix: Clustering. meat, block, shape, cup, dustpan, broom, tap, drawer, stick.
